An Algorithm-Hardware Co-Optimized Framework for Accelerating N:M Sparse Transformers

The Transformer has been an indispensable staple in deep learning. However, for real-life applications, it is very challenging to deploy efficient Transformers due to immense parameters and operations of models. To relieve this burden, exploiting sparsity is an effective approach to accelerate Transformers. Newly emerging Ampere GPUs leverage a 2:4 sparsity pattern to achieve model acceleration, while it can hardly meet the diverse algorithm and hardware constraints when deploying models. By contrast, we propose an algorithm-hardware co-optimized framework to flexibly and efficiently accelerate Transformers by utilizing general N:M sparsity patterns. (1) From algorithm perspective, we propose a sparsity inheritance mechanism along with an inherited dynamic pruning (IDP) method to obtain a series of N:M sparse candidate Transformers rapidly. A model compression scheme is further proposed to significantly reduce the storage requirement for deployment. (2) From hardware perspective, we present a flexible and efficient hardware architecture, namely STA, to achieve significant speedup when deploying N:M sparse Transformers. STA features not only a computing engine unifying both sparse-dense and dense-dense matrix multiplications with high computational efficiency but also a scalable softmax module eliminating the latency from intermediate off-chip data communication. Experimental results show that compared to other methods, N:M sparse Transformers, generated using IDP, achieves an average of 6.7% improvement on accuracy with high training efficiency. Moreover, STA can achieve 14.47x and 11.33x speedup compared to Intel i9-9900X and NVIDIA RTX 2080 Ti, respectively, and perform 2.00-19.47x faster inference than the state-of-the-art FPGA-based accelerators for Transformers.

==> 0-bio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.2in,clip,keepaspectratio]{figs/TVLSI-bio-fangchao.pdf}}]{Chao Fang}
received the B.S. degree in Tianjin University, Tianjin, China, in 2019. He is currently pursuing the Ph.D. degree with Nanjing University, Nanjing, China.

His current research interests include model compression algorithm and domain-specific accelerator design for machine learning.
 \vspace{-0.4in}
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.2in,clip,keepaspectratio]{figs/TVLSI-bio-ajzhou.jpeg}}]{Aojun Zhou}
received the M.S. degree in National Laboratory of Pattern Recognition (NLPR), Institute of Automation Chinese Academy of Science (CASIA), China. in 2019. He is currently working toward the PhD degree in the Department of Electronic Engineering, The Chinese University of Hong Kong. 
His research interests include deep learning and computer vision.
 \vspace{-0.4in}
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage


\begin{IEEEbiography}[{\includegraphics[width=1.25in,height=1.25in,clip,keepaspectratio]{figs/TVLSI-bio-zfwang.jpg}}]{Zhongfeng Wang}
(M'00-SM'05-F'16) received both the B.E. and M.S. degrees in the Dept. of Automation at Tsinghua University, Beijing, China, in 1988 and 1990, respectively. He obtained the Ph.D. degree from the University of Minnesota, Minneapolis, in 2000. He has been working for Nanjing University, China, as a Distinguished Professor since 2016. Previously he worked for Broadcom Corporation, California, from 2007 to 2016 as a leading VLSI architect. Before that, he worked for Oregon State University and National Semiconductor Corporation.

Dr. Wang is a world-recognized expert on Low-Power High-Speed VLSI Design for Signal Processing Systems. He has published over 200 technical papers with multiple best paper awards received from the IEEE technical societies, among which is the VLSI Transactions Best Paper Award of 2007. He has edited one book VLSI and held more than 20 U.S. and China patents. In the current record, he has had many papers ranking among top 25 most (annually) downloaded manuscripts in IEEE Trans. on VLSI Systems. In the past, he has served as Associate Editor for IEEE Trans. on TCAS-I, T-CAS-II, and T-VLSI for many terms. He has also served as TPC member and various chairs for tens of international conferences. Moreover, he has contributed significantly to the industrial standards. So far, his technical proposals have been adopted by more than fifteen international networking standards. In 2015, he was elevated to the Fellow of IEEE for contributions to VLSI design and implementation of FEC coding. His current research interests are in the area of Optimized VLSI Design for Digital Communications and Deep Learning.
\end{IEEEbiography}


% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
    
    

==> src/0-abstr.tex <==
% As a general rule, do not put math, special symbols or citations
% in the abstract or keywords.
\begin{abstract}
The Transformer has been an indispensable staple in deep learning. 
% [TODO] 这句话需要斟酌。
% However, the great storage and computation requirements of Transformer models make it challenging to realize efficient deployment for Transformer-based applications.
% However, Transformer itself usually has a large amount of storage and computing requirements, which makes it very challenging to realize efficient deployment for real-life applications.
However, for real-life applications, it is very challenging to deploy efficient Transformers due to immense parameters and operations of models.
% However, immense parameters and operations. of models make it very challenging to deploy efficient Transformers for real-life applications.
% To relieve this burden, exploiting sparsity is a powerful tool for accelerating Transformers.
To relieve this burden, exploiting sparsity is an effective approach to accelerate Transformers.
% Newly emerging Ampere GPUs leverage a \textit{2:4} sparsity pattern to achieve model acceleration, but this solution can hardly meet the diverse needs of consumers when deploying models.
Newly emerging Ampere GPUs leverage a \textit{2:4} sparsity pattern to achieve model acceleration, while it can hardly meet the diverse algorithm and hardware constraints when deploying models.
% [TODO] Chao Fang: 这句话可能有点问题。
By contrast, we propose an algorithm-hardware co-optimized framework to flexibly and efficiently accelerate Transformers by utilizing general \textit{N:M} sparsity patterns.
% By contrast, we propose an algorithm-hardware co-optimized framework to accelerate Transformers by utilizing general \textit{N:M} sparsity patterns, which is more flexible and efficient to support various architectural settings.
(1) From algorithm perspective, we propose a sparsity inheritance mechanism along with inherited dynamic pruning (IDP) to obtain a series of \textit{N:M} sparse candidate Transformers rapidly.
A model compression scheme is further proposed to significantly reduce the storage requirement for deployment.
% To address this issue, we present an algorithm-hardware co-optimization solution in this paper.
% [TODO] 这句话说的不够好，存在问题，没有把硬件的部分给写出来。
% Our solution takes as input a well-trained dense Transformer, and generates as output a highly compressed $N$:$M$ sparse Transformer, which maintains similar accuracy while achieving dramatic reduction on the storage and computing compared to the dense one. 
% To be precise, 
% [TODO] 这个 which 从句想个办法替换掉，太多这样的从句了。
% At the algorithm level, we propose an incremental dynamic pruning method for $N$:$M$ sparsity pattern, which greatly reduces the amount of parameters of the Transformer model.
% Then, a parameter compression scheme is proposed for the $N$:$M$ sparse Transformer to significantly reduce the storage requirement for deployment.
% At the hardware level, we design a flexible hardware generator to support deployments targeting various $N$:$M$ sparse patterns, Transformer-based models, and hardware platforms.
(2) From hardware perspective, we present a flexible and efficient hardware architecture, namely STA, to achieve significant speedup when deploying \textit{N:M} sparse Transformers.
STA features not only a computing engine unifying both sparse-dense and dense-dense matrix multiplications with high computational efficiency but also a scalable softmax module eliminating the latency from intermediate off-chip data communication.
Experimental results show that compared to other methods, \textit{N:M} sparse Transformers, generated using IDP, achieves an average of $6.7\%$ improvement on accuracy with high training efficiency.
Moreover, STA can achieve $14.47\times$ and $11.33\times$ speedup compared to Intel i9-9900X and NVIDIA RTX 2080 Ti, respectively, and perform $ 2.00 \sim 19.47 \times $  faster inference than the state-of-the-art FPGA-based accelerators for Transformers.
\end{abstract}

% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
Algorithm-hardware co-design, Transformer, hardware accelerator, pruning, model compression.
\end{IEEEkeywords}


==> src/0-ack.tex <==
% use section* for acknowledgment
\section*{Acknowledgment}

We would like to sincerely thank our reviewers for their valuable feedback.

==> src/0-bio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.2in,clip,keepaspectratio]{figs/TVLSI-bio-fangchao.pdf}}]{Chao Fang}
received the B.S. degree in Tianjin University, Tianjin, China, in 2019. He is currently pursuing the Ph.D. degree with Nanjing University, Nanjing, China.

His current research interests include model compression algorithm and domain-specific accelerator design for machine learning.
 \vspace{-0.4in}
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.2in,clip,keepaspectratio]{figs/TVLSI-bio-ajzhou.jpeg}}]{Aojun Zhou}
received the M.S. degree in National Laboratory of Pattern Recognition (NLPR), Institute of Automation Chinese Academy of Science (CASIA), China. in 2019. He is currently working toward the PhD degree in the Department of Electronic Engineering, The Chinese University of Hong Kong. 
His research interests include deep learning and computer vision.
 \vspace{-0.4in}
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage


\begin{IEEEbiography}[{\includegraphics[width=1.25in,height=1.25in,clip,keepaspectratio]{figs/TVLSI-bio-zfwang.jpg}}]{Zhongfeng Wang}
(M'00-SM'05-F'16) received both the B.E. and M.S. degrees in the Dept. of Automation at Tsinghua University, Beijing, China, in 1988 and 1990, respectively. He obtained the Ph.D. degree from the University of Minnesota, Minneapolis, in 2000. He has been working for Nanjing University, China, as a Distinguished Professor since 2016. Previously he worked for Broadcom Corporation, California, from 2007 to 2016 as a leading VLSI architect. Before that, he worked for Oregon State University and National Semiconductor Corporation.

Dr. Wang is a world-recognized expert on Low-Power High-Speed VLSI Design for Signal Processing Systems. He has published over 200 technical papers with multiple best paper awards received from the IEEE technical societies, among which is the VLSI Transactions Best Paper Award of 2007. He has edited one book VLSI and held more than 20 U.S. and China patents. In the current record, he has had many papers ranking among top 25 most (annually) downloaded manuscripts in IEEE Trans. on VLSI Systems. In the past, he has served as Associate Editor for IEEE Trans. on TCAS-I, T-CAS-II, and T-VLSI for many terms. He has also served as TPC member and various chairs for tens of international conferences. Moreover, he has contributed significantly to the industrial standards. So far, his technical proposals have been adopted by more than fifteen international networking standards. In 2015, he was elevated to the Fellow of IEEE for contributions to VLSI design and implementation of FEC coding. His current research interests are in the area of Optimized VLSI Design for Digital Communications and Deep Learning.
\end{IEEEbiography}


% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
    
    

==> src/0-ccls.tex <==
\section{Conclusion}
In this paper, we present a flexible, agile, and efficient framework for deploying \textit{N:M} sparse Transformers, which is benefited from both algorithm and hardware optimizations, making it practical to significantly accelerate Transformer-based models on diverse FPGA devices.
At the algorithm level, we propose a sparsity inheritance mechanism and a inherited dynamic pruning (IDP) method to obtain a series of \textit{N:M} sparse Transformers with high accuracy. 
A further proposed compression scheme greatly reduces the storage requirements of models.
At the hardware level, we present a flexible and efficient architecture, namely STA, to accelerate \textit{N:M} sparse Transformers.
STA is composed of a computing core, DMME, that unifies both sparse and dense intensive matrix multiplications in \textit{N:M} sparse Transformers, and a scalable softmax module, which eliminates intermediate off-chip data accesses.
The experimental results show that \textit{N:M} sparse Transformers generated by IDP achieves an average of $6.7\%$ improvement in accuracy over the state-of-the-art methods.
STA implementation significantly outperforms CPU, GPU, and prior FPGA-based Transformer accelerators in terms of latency, throughput, energy efficiency, and MAC efficiency, showing its significant potential in applications using Transformer-based models.

==> src/0-info.tex <==
%
% paper title
% Titles are generally capitalized except for words such as a, an, and, as,
% at, but, by, for, in, nor, of, on, or, the, to and up, which are usually
% not capitalized unless they are the first or last word of the title.
% Linebreaks \\ can be used within to get better formatting as desired.
% Do not put math or special symbols in the title.
% \title{面向边缘计算平台的 \\ Transformer模型加速框架}
% \title{Accelerating Sparse Transformers with Algorithm-Hardware Co-Optimization}
\title{An Algorithm-Hardware Co-Optimized Framework for Accelerating \textit{N:M} Sparse Transformers}
%
%

% author names and IEEE memberships
% note positions of commas and nonbreaking spaces ( ~ ) LaTeX will not break
% a structure at a ~ so this keeps an author's name from being broken across
% two lines.
% use \thanks{} to gain access to the first footnote area
% a separate \thanks must be used for each paragraph as LaTeX2e's \thanks
% was not built to handle multiple paragraphs
%

\author{Chao~Fang,~\IEEEmembership{Graduate~Student~Member,~IEEE,}
        Aojun~Zhou, 
        and~Zhongfeng~Wang,~\IEEEmembership{Fellow,~IEEE}% <-this % stops a space
\thanks{This work was supported in part by the National Natural Science Foundation of China under Grant 62174084, 62104097 and in part by the High-Level Personnel Project of Jiangsu Province under Grant JSSCBS20210034, the Key Research Plan of Jiangsu Province of China under Grant BE2019003-4. \textit{(Corresponding author: Zhongfeng Wang.)}}
\thanks{C. Fang and Z. Wang are with the School of Electronic Science and Engineering, Nanjing University, Nanjing 210008, China (e-mail: fantasysee@smail.nju.edu.cn;
zfwang@nju.edu.cn).}% <-this % stops a space
\thanks{A. Zhou is with CUHK-Sensetime Joint Lab, CUHK, Hong Kong, China (e-mail: aojunzhou@gmail.com).}% <-this % stops a space
% \thanks{Manuscript received April 19, 2005; revised August 26, 2015.}
}

% note the % following the last \IEEEmembership and also \thanks - 
% these prevent an unwanted space from occurring between the last author name
% and the end of the author line. i.e., if you had this:
% 
% \author{....lastname \thanks{...} \thanks{...} }
%                     ^------------^------------^----Do not want these spaces!
%
% a space would be appended to the last name and could cause every name on that
% line to be shifted left slightly. This is one of those "LaTeX things". For
% instance, "\textbf{A} \textbf{B}" will typeset as "A B" not "AB". To get
% "AB" then you have to do: "\textbf{A}\textbf{B}"
% \thanks is no different in this regard, so shield the last } of each \thanks
% that ends a line with a % and do not let a space in before the next \thanks.
% Spaces after \IEEEmembership other than the last one are OK (and needed) as
% you are supposed to have spaces between the names. For what it is worth,
% this is a minor point as most people would not even notice if the said evil
% space somehow managed to creep in.



% The paper headers
\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2015}%
{Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Journals}
% The only time the second header will appear is for the odd numbered pages
% after the title page when using the twoside option.
% 
% *** Note that you probably will NOT want to include the author's ***
% *** name in the headers of peer review papers.                   ***
% You can use \ifCLASSOPTIONpeerreview for conditional compilation here if
% you desire.




% If you want to put a publisher's ID mark on the page you can do it like
% this:
%\IEEEpubid{0000--0000/00\$00.00~\copyright~2015 IEEE}
% Remember, if you use this you must call \IEEEpubidadjcol in the second
% column for its text to clear the IEEEpubid mark.



% use for special paper notices
%\IEEEspecialpapernotice{(Invited Paper)}

% make the title area
\maketitle

==> src/0-ref.tex <==
% Can use something like this to put references on a page
% by themselves when using endfloat and the captionsoff option.
\ifCLASSOPTIONcaptionsoff
  \newpage
\fi



% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
\bibliography{src/ref.bib}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
% \begin{thebibliography}{1}

% \bibitem{IEEEhowto:kopka}
% H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
%   0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

% \end{thebibliography}

==> src/1-sec-intro.tex <==
\section{Introduction}

% \begin{itemize}
%     \item % 介绍 Transformer 模型的应用。
%     \item % 介绍当前 Transformer 模型在边缘平台部署时候遇到的挑战。
%     \item % 介绍现今存在的一些具体方案，是如何做的，还存在哪些不足。
%     \item % 由此引出自己的工作，一个 Transformer 模型加速的边缘平台部署框架。该框架分别包含算法上的稀疏以及硬件上的设计。每个部分分别具有什么优势。
% \end{itemize}
\IEEEPARstart{T}{ransformer-based} networks are a formidable force in deep learning \cite{tay2020efficient}.
Tremendous impact in many fields, such as neural machine translation \cite{song2020alignment}, language understanding \cite{kenton2019bert}, and image processing \cite{dosovitskiy2020image}, has been made since the innovation of Transformers. 
Nevertheless, the impressive performance of Transformers comes with heavy computing and memory costs, which become a significant barrier to the efficient deployment of Transformer-based applications.
Notably, BERT, a representative Transformer-based model \cite{kenton2019bert},  requires \textit{440MB} memory and over \textit{176G} floating-point operations. 
% Moreover, it takes 8.13 ms to complete the forward pass of the Transformer-base model on the NVIDIA RTX 2080 Ti GPU with a thermal design power (TDP) of 250W. 
Such severe requirements on memory and computation make it critical to find an efficient solution for deploying Transformers.

\begin{figure} [htbp] 
	\centering
	\includegraphics[width=0.42\textwidth]{figs/r1-TVLSI-1-intro-cmp-new.pdf}
	\caption{\RoundOne{Accelerating \textit{\textit{N:M}} sparse Transformer-based models (a) using modern Ampere GPUs and (b) using diverse FPGAs with our framework. 
	Compared to (a), (b) can generate a series of \textit{\textit{N:M}} sparse Transformers along with the dedicated accelerators for efficient model deployment.}
	} 
	\label{fig:sol_cmp}
\end{figure}

% [Note] Chao Fang: 目前来看，这里的承接貌似有些生硬。主要是 Dedicated Accelerator 的部分上文没有提到，应该如何理顺这个逻辑呢？
% \AJ{Sparsity is an important feature to improve the efficiency of DNNs deployment in dedicated accelerators.} 
Sparsity is an important feature that can be utilized to improve the efficiency of DNNs deployment in dedicated accelerators.
% [Note] Chao Fang: 这里的逻辑不好。
%\FC{
In the pioneering works, OPTIMUS \cite{park2020optimus} and EdgeBERT \cite{tambe2021edgebert}, the latest ASIC accelerators, leverage unstructured sparsity to realize efficient deployment for Transformers.
% \AJ{previous works[xxxx] leverage unstructured sparsity to xxx.} 
Nevertheless, it is hard to predict the unstructured sparsity in advance, and therefore the acceleration performance can be greatly dragged.
%}
% \AJ{ 
% ??drawback .. NV..???. 
% [TODO] Chao Fang: 这句话的逻辑有问题，需要重新写。
Recent studies \cite{zhou2021learning} demonstrate deep neural networks leveraging \textit{N:M} fine-grained structured sparsity, where \textit{N} out of \textit{M} parameters are zeros for every continuous \textit{M} parameters, can achieve comparable performance over those leveraging unstructured sparsity \cite{sun2021dominosearch}. 
% N:M weight pruning where N out of M weights are zeros for every continuous M weights. 
% There is limited choice
% \FC{
However, it is significantly restricted to accelerate \textit{N:M} sparse networks on current hardware platforms.
As shown in Fig.~\ref{fig:sol_cmp}~(a), the only existing solution is \textit{ASP with Ampere GPUs} that focuses on the middle-level (\textit{2:4}), i.e., 50\%, sparse ratio. 
Based on our experiments, a heavy Transformer can be dramatically slimmed by weight pruning with the aggressive \textit{N:M} pattern, e.g., \textit{2:8} or \textit{1:8}, achieving a considerable reduction in the amount of both parameters and operations.
% [TODO] Chao Fang: 下面这句话需要重新写。
The only choice of uniform \textit{2:4} sparsity limits performance when deploying Transformer-based models, making it inflexible to meet different hardware constraints (e.g., latency, energy).
% Actually, consumers have different specifications of model deployment in their own way.
% Consumers usually have different specifications of model deployment in their way.
% Some may prioritize model accuracy, and some may focus on inference latency.
% Some may have a device with abundant hardware resources, while others may have a resource-constrained device.
% We believe that,
Compared with the uniform \textit{2:4} sparsity, the more flexible general \textit{N:M} sparsity in real applications can satisfy various algorithm and hardware constraints under different deployment scenarios.
% We believe that, compared with the uniform \textit{2:4} sparsity, the more flexible general \textit{N:M} sparsity in real applications can truly meet the needs of diverse consumers to realize personalized deployment.
% We believe that general \textit{N:M} sparsity pattern is more flexible in real applications over uniform 2:4 sparsity pattern, and can 
% }
% Actually, the heavy Transformer can be significantly sparsified by weight pruning (e.g., [xxx]), and    
% However, There lack of an integrated framework to investigate the deployment of Transformer with general \textit{N:M} sparse pattern.
However, there is currently a lack of an integrated framework to investigate the deployment of Transformer with general \textit{N:M} sparse patterns. 
% \FC{
To bridge this gap, as presented in Fig.~\ref{fig:sol_cmp}~(b), we propose an algorithm-hardware co-optimized framework for accelerating \textit{N:M} sparse Transformers, which addresses two significant issues: \textbf{1). how to produce a series of \textit{N:M} sparse Transformers in an efficient way; 2). how to design a flexible and efficient dedicated architecture for \textit{N:M} sparse Transformers on diverse FPGA platforms.}
% In this paper, we present our FPGA-based framework with algorithm-hardware co-optimizaiton to bridge this gap.
% Our framework addresses two significant issues: \textbf{(1). how to produce a series of \textit{N:M} sparse Transformers in an efficient way. (2). how to design a flexible and efficient dedicated architecture for \textit{N:M} sparse Transformers on diverse FPGA platforms.}
% Our framework, the producer in Fig.~\ref{fig:sol_cmp}~(b), takes additional user-defined specifications as input. 
% Then it generates a winner \textit{N:M} sparse Transformer among diverse candidates with arbitrary \textit{N:M} pattern, along with the dedicated sparse Transformer accelerator.
% }
% The framework should address two significant questions: \textbf{(1). how to produce arbitrary \textit{N:M} sparse Transformer models in an efficient way. (2). can we leverage different \textit{N:M} configurations to achieve the efficiency-accuracy trade-off on FPGA platforms}.
% Our framework addresses two significant issues: \textbf{(1). how to produce a series of \textit{N:M} sparse Transformers in an efficient way. (2). how to design a flexible and efficient dedicated architecture for \textit{N:M} sparse Transformers on diverse FPGA platforms.}
% }  

% [Note] Chao Fang: 这里还需要插入一段解释 Fig. 1.
%\AJ{Therefore, in this paper, we propose an integrated Algorithm-Hardware Co-design framework to study the deployment of general \textit{N:M} fine-grained structured sparse Transformers. Firstly, we propose a novel algorithm xxxx that  progressively produces a series of \textit{N:M}-pattern-based sparse models under different sparse ratio (e.g., 2:8, 1:8). Secondly, we design xxx, which can }.

% \AJ{
Although advanced optimization algorithms ASP\cite{mishra2021accelerating} and SR-STE\cite{zhou2021learning} can maintain the middle-level (\textit{2:4}) sparsity via static and dynamic fine-tuning, we observe existing methods degrade the performance significantly under high sparse ratio (e.g., $\geq 75\%$). 
In addition, the ASP and SR-STE schemes leverage single-shot magnitude-based pruning for a specified hyper-parameter \textit{N} and \textit{M}.  
This traditional recipe results in a significant performance drop with a higher sparse ratio and restricts the deployment of flexible \textit{N:M} sparse models on the FPGA platform. 
To overcome the aforementioned problems, we propose a sparsity inheritance mechanism, which increases the sparsity progressively to enable efficient searching for $N$:$M$ sparse Transformers under various sparsity configurations (e.g., \textit{2:8}, \textit{1:8}). 
We also propose a pruning method, namely inherited dynamic pruning (IDP), which shrinks pre-pruning models progressively, and the convergent pre-pruning initialized models can aid in the convergence of the following sub-networks. 
Extensive experiments are conducted on Transformer-based models, showing that models generated by IDP with the sparsity inheritance mechanism have superior performance on various sparsity ratios than those using the ASP and SR-STE.
% \RoundOne{
Moreover, for efficient model deployment, we apply a simple but effective bitmap-based compression scheme, which dramatically reduce the storage requirements for \textit{N:M} sparse Transformers.
% }
% [TODO] Chao Fang: 压缩的部分是否还要提一嘴？
% }

% To provide a better initialization and transfer the knowledge of the lower sparsity to the higher sparsity, we propose a sparsity inheritance mechanism, which increases the sparsity progressively to enable efficient searching for $N$:$M$ sparse Transformers under various sparsity configurations.

% \FC{
To enable flexible and efficient deployment on various FPGA devices, we design a highly configurable dedicated accelerator for \textit{N:M} sparse Transformers, namely STA.
STA fully explores the parallelism of Transformers in three aspects, including head parallelism, row parallelism, and column parallelism, which significantly improves computational efficiency.
It features two computing cores, a diverse matrix multiplication (MatMul) engine, called DMME, and a scalable softmax module, both of which are highly configurable.
% [TODO] Chao Fang
% Two types of MatMuls dominate operations of \textit{N:M} sparse Transformers. 
Operations of \textit{N:M} sparse Transformers are dominated by two types of MatMuls.
One is the sparse-dense MatMul with \textit{N:M} sparse network parameters, and the other is dense-dense MatMul free of parameters.
DMME performs both sparse-dense and dense-dense MatMuls on-the-fly, and achieves much higher computational efficiency over the prior work \cite{lu2020hardware} under both modes.
Especially for sparse-dense MatMul, DMME only performs operations related to those remaining non-zero parameters, which greatly improves computational efficiency.
The scalable softmax module can perform the softmax function in Transformers. 
It keeps all the intermediate results fully local, eliminating latency from intermediate off-chip data communication.
According to the given architectural settings, STA can be rapidly implemented on FPGAs to realize efficient deployment for specific \textit{N:M} sparse Transformers.
% }

% The contribution of this paper can be summarized as follows.
% Our contributions are summarized as follows.
To summarize, the contributions of our paper are as follows:
% \FC{
\begin{itemize}
    \item To our best knowledge, this is the first work that presents an algorithm-hardware co-optimized framework to systematically study the efficiency of fine-grained \textit{N:M} sparse Transformers on FPGA. The proposed framework can adjust to diverse hardware constraints for flexible and efficient model deployment.
    % \item An algorithm-hardware co-optimization framework is proposed for flexible and efficient model deployment of \textit{N:M} sparse Transformers on FPGA platforms. The framework can implement personalized model deployment for diverse consumers according to their various needs.
    \item To generate a series of \textit{N:M} sparse Transformers simultaneously, we propose a sparsity inheritance mechanism along with the inherited dynamic pruning (IDP) algorithm, which can significantly achieve about $6.7\%$ accuracy improvement of Transformers under high sparsity compared with state-of-the-art methods.
    \item We present a simple but effective bitmap-based compression scheme for \textit{N:M} sparse Transformers compared to multiple sparse indexing formats, which dramatically reduces the storage requirements up to $5.33 \times$.
    % [Note] Chao Fang: 感觉这里写的不够好。
    % \item A sparsity inheritance mechanism is proposed to produce arbitrary \textit{N:M} sparse Transformer models with high quality on model accuracy over the existing methods. In addition, a compression scheme for \textit{N:M} sparse models is proposed, which significantly reduces the storage requirements when deploying models on FPGA devices.
    \item We propose a dedicated hardware architecture, namely STA, to realize flexible and efficient deployment of \textit{N:M} sparse Transformers. It features two novel hardware modules handling intensive operations of Transformers, including a diverse matrix multiplication engine (DMME) that unifies dense and sparse MatMul operations in high computational efficiency, and a scalable softmax module to avoid frequent off-chip memory accesses.
    % \item A dedicated hardware architecture, namely STA, is proposed to realize efficient deployment of \textit{N:M} sparse Transformers. It features a diverse matrix multiplication engine (DMME) that unifies dense and sparse MatMul operations in high computational efficiency, and a scalable softmax module to avoid frequent off-chip memory accesses. 
    \item Extensive experiments have been conducted on four NLP tasks and four Transformer-based models to evaluate the effectiveness of the proposed framework, which achieves up to $19.47\times$ speedup over Intel i9-9900X, NVIDIA RTX 2080 Ti, and prior FPGA-based accelerators for Transformers.
    % \item We evaluate IDP on four NLP tasks and STA on four Transformer-based models, and find that our proposed framework achieves up to $19.47\times$ speedup over Intel i9-9900X, NVIDIA RTX 2080 Ti, and prior FPGA-based accelerators for Transformers.
    %\item  [Note] Chao Fang: 是否需要把实验的结果也作为 contrib 呢？
\end{itemize}
% }
% \begin{itemize}
%     \item We present an algorithm-hardware co-optimization solution for efficient deployment of Transformer-based model on real-life applications. 
%     \item We propose an incremental dynamic pruning (IDP) method to obtain $N$:$M$ sparse Transformers with significant reduction on parameters. 
%     \item We also develop a model compression scheme on $N$:$M$ sparse Transformers to achieve substantial saving on storage and computing for deployment.
%     \item We develop an efficient hardware generator to support flexible and diverse requirements on model deployment. 
%     \item For the generated accelerator, we elaborately design not only a novel unified computing engine for sparse-dense and dense-dense matrix multiplications with high hardware utilization, but also a scalable softmax module to eliminate the off-chip data transfer for the intermediate softmax operator.
%     \item We evaluate 
% \end{itemize}

The rest of this paper is organized as follows: Section~\ref{sec:bkg} presents an overview of Transformers, and state-of-the-art works for accelerating Transformers with innovations on hardware architecture. 
Section~\ref{sec:overview} introduces the workflow of our proposed algorithm-hardware co-optimization framework.
Section~\ref{sec:algo} and Section~\ref{sec:hwarch} elaborate optimizations on pruning algorithm and hardware architecture, respectively.
Comprehensive experimental results are presented in Section~\ref{sec:res} to show significant potential of our proposed co-optimization framework in Transformer-based applications.

==> src/2-sec-bkg.tex <==
\section{Background and Motivation} \label{sec:bkg}

In this section, we provide an overview of key structures in Transformers, and review related work on hardware accelerators for Transformers.

% \begin{itemize}
% 	\item % 简单介绍 Transformer 的模型结构。（是否应该在该章节展示一些数据介绍 Transformer 的计算瓶颈？）介绍一下算子分类。最好还要有相应的 Latency breakdown，展示 Transformer 各个算子的运算时间。
% 	\item % 介绍当前稀疏 Transformer 的研究现状，包括算法上的进展以及硬件上的进展。这里需要对不同的稀疏 pattern 进行总结对比。基于以上研究现状，进行总结，谈他们存在的不足，突出软硬协同一体的优势。
% \end{itemize}

\subsection{Transformer Overview}

The key architectures of the Transformer \cite{vaswani2017attention} are characterized by a multi-head attention (MHA) residual block (ResBlock) and a position-wise feed-forward network (FFN) ResBlock.
Fig.~\ref{fig:model_overview}~(a) and (b) illustrate the inner structures of MHA and FFN ResBlocks, respectively.
The input and output of the FFN ResBlock are connected by a residual connector. 
And two linear transformation modules along with a activation function are inside the FFN ResBlock. 
The structure of MHA ResBlock is more complicated. 
The inputs of MHA ResBlock are split into multiple parallel heads with corresponding linear projection at first. 
Then the results are as input fed into the attention mechanism in parallel, and finally, the results of attention heads are concatenated together and passed into a
linear layer to obtain the output linear projection. 
Note that the attention mechanism is totally different from the linear layer,
performing parameter-free MatMuls. 
Thus, the computing engine for Transformers is required to support both sparse and dense MatMuls even though sparsity is introduced to parameters.
The residual connector of FFN ResBlock is organized the same as the FFN ResBlock.

\begin{figure} [htbp] 
	\centering
	\includegraphics[width=0.48\textwidth]{figs/TVLSI-2-bkg-model_key_structure.pdf}
	\caption{The operations in (a) the MHA ResBlock and (b) the FFN ResBlock under \textit{\textit{N:M}} sparsity pattern. Both Resblocks are the key structures of the Transformer. (c) An illustration of \textit{2:4} sparse parameters in a linear layer.} 
	\label{fig:model_overview}
\end{figure}
% The key architecture of the Transformer \cite{vaswani2017attention} is presented in Fig.~\ref{fig:model_overview} (a).
% It is formed by stacking multiple encoder and decoder sublayers. 
% Both encoder and decoder are characterized by a position-wise feed-forward network (FFN) residual block (ResBlock) and a multi-head attention (MHA) ResBlock.  
% Fig.~\ref{fig:model_overview} (b) and (c) illustrate the inner architecture of FFN and MHA ResBlocks, respectively.
% % 分别一下 FFN ResBlocks 和 MHA ResBlocks 的结构
% The input and output of the FFN ResBlock are connected by a residual connector and a layer normalization (LayerNorm) module.
% And two linear transformation modules along with a ReLU activation function are inside the FFN ResBlock.
% The structure of MHA ResBlock is more complicated.
% The inputs of MHA ResBlock are split into multiple parallel heads with corresponding linear projection at first. 
% Then the results are as input fed into the attention mechanism in parallel, and finally, the results of attention heads are concatenated together and passed into a linear layer to obtain the output linear projection.
% Note that the attention mechanism is totally different from the linear layer, performing parameter-free MatMuls.
% % Note that the attention mechanism performs parameter-free matrix multiplication, which is different from the linear layer.
% The residual connector and LayerNorm module of FFN ResBlock are organized the same as the FFN ResBlock.
% 再提一下两种 LayerNorm 的形式
% The position of LayerNorm in ResBlocks indicates that there are two kinds of basic Transformer structures, \textit{i.e.}, Pre-LN and Post-LN Transformers \cite{liu2020very, liu2020understanding, xiong2020layer}. 

\subsection{Recent Advances for Transformer Acceleration}

% 学习 EdgeBERT 的 Related Works 的写法。先说 加速器的设计进展，然后提Transformer的进展
Extensive research has concentrated on the design of high-performance and energy-efficient DNN hardware accelerators \cite{wu2021swm, colleman2021high, yantir2021imca, yin2019vesti, paulin2021rnn, fang2021accelerating, yu2020uni, zhu2020efficient, moreno2020analysis, lian2019high, kala2019high, xie2021efficient, albericio2016cnvlutin, chen2016eyeriss, liu2016cambricon, liu2020systolic, parashar2017scnn}.
% The interest in design auto-generation arises as well due to the trends that these aforementioned accelerators are increasingly deployed at all computing scales.
% As these accelerators are increasingly deployed at all computing scales, there is additional interest in the hardware community to automatically generate designs.
However, most of these works focus on CNN and RNN computations, and not as much scrutiny has been given to accelerating Transformer-based networks with self-attention mechanisms.
% [Note] Chao Fang: 这里 self-attention 并没有进行解释。上面这句话是需要修改的。

As a pioneer work, \cite{lu2020hardware} proposed a dense systolic array accelerator along with the partitioning scheme for FPGA-based acceleration of Transformers.
Moreover, FTRANS \cite{li2020ftrans} exploited block-circulant matrix-based weight representation for Transformer acceleration. 
However, both of them fail to utilize the sparsity of parameters in Transformers, thereby limiting the speedup of model deployment. 
A$^{3}$ \cite{ham2020a3}, SpAtten \cite{wang2021spatten}, and Sanger \cite{lu2021sanger} merely focused on the speedup potential for the sparse attention mechanism, all of which can hardly satisfy the needs of agile and efficient deployment of Transformer models. 
OPTIMUS \cite{park2020optimus} and EdgeBERT \cite{tambe2021edgebert} holistically accelerate Transformers with unstructured sparse matrix multiplications and save energy by skipping the computations related to those zero-value parameters.
Nevertheless, the unstructured sparsity leads to irregular data access, making both designs suffer low computational efficiency.
\cite{peng2021accelerating} exploited the coarse-grained block-based sparsity pattern for accelerating Transformers, while this sparsity pattern is so coarse that the models can hardly achieve a considerable sparsity ratio with acceptable accuracy. 
% Therefore, it is hard to realize significant acceleration.
% And therefore, the limited compression ratio of models on the parameters and operations make it hard to realize significant acceleration.

% \textbf{====== TODO ======}

% \begin{itemize}
% 	\item 
% 	% [TODO] 这句话有问题，可能需要修改
% 	\item FTRANS \cite{li2020ftrans} adopted a block-circulant matrix-based representation for parameter compression, and introduced frequency domain acceleration.
% 	\item A$^{3}$ \cite{ham2020a3}, SpAtten \cite{wang2021spatten}, and Sanger \cite{lu2021sanger} merely focused on the speedup potential for the sparse attention mechanism.
% 	\item OPTIMUS \cite{park2020optimus} and EdgeBERT \cite{tambe2021edgebert}
% 	\item \cite{peng2021accelerating} exploited the coarse-grained block-based sparsity pattern.
% \end{itemize}

% \textbf{====== TODO ======}
% \FC{
In summary, it is hard for all these works to achieve satisfying speedup and efficiency of Transformer deployment due to the lack of attention to model sparsity, limited sparse potential exploration on the whole Transformer models, or restricted computational efficiency for sparse Transformers.
% In summary, the lack of attention to model sparsity, limited sparse potential exploration on the whole Transformer models, or restricted computational efficiency for sparse Transformers, make it hard to achieve satisfying speedup for the Transformer-based model deployment.
% [Note] Chao Fang: 这里开始写我们工作的 highlight，重点解决了以上工作的哪些问题。
To address above issues, this work presents an algorithm-hardware co-optimization framework to realize flexible and efficient deployment of Transformers by leveraging general \textit{N:M} sparsity patterns.
For algorithm optimization, we focus on how to generate a series of \textit{N:M} sparse Transformers in high quality and efficiency.
For hardware optimization, we concentrate on designing a flexible and efficient dedicated architecture that can accelerate \textit{N:M} sparse Transformers with high computational efficiency.
% For hardware optimization, we concentrate on the design of efficient dedicated accelerator for \textit{N:M} sparse Transformers, which can achieve high computational efficiency.
% }

==> src/3-sec-overview.tex <==
\begin{figure*} [ht] 
	\centering
	\includegraphics[width=0.92\textwidth]{figs/r1-TVLSI-3-overview-workflow-complicated.pdf}
	\caption{\RoundOne{The workflow of our proposed algorithm-hardware co-optimized framework. At the algorithm level, \textit{N:M} sparse Transformers can be rapidly generated by inherited dynamic pruning, and significantly compressed for further deployment. At the hardware level, the dedicated accelerator, STA, is implemented on the FPGA platform to accelerate the deployed \textit{N:M} sparse Transformer.}}
	\label{fig:workflow}
\end{figure*}

\section{Overview of Co-optimization} \label{sec:overview}

% \begin{itemize}
% 	\item % 框架的设计目标。
% 	\item % 框架的组成部分，包括算法上和硬件上。
% 	\item % 各个组成部分的技术优势。最后获得整个框架的设计优势。
% \end{itemize}

% For agile and efficient deployment of Transformers, we propose an algorithm-hardware co-optimization framework.
% [TODO] 这里如何总结，是不是要模仿 Sanger 的写法？
% 
To achieve agile and efficient deployment of Transformers, we propose an algorithm-hardware co-optimized framework.
The overview of our framework is presented in Fig.~\ref{fig:workflow}.
% The framework serves consumers that have various FPGA devices.
% According to the specific requirements of consumers, our framework can quickly obtain the required \textit{N:M} sparse Transformer model with high quality, and provide corresponding Transformer accelerators on FPGA devices to realize efficient model deployment.
According to the given specific requirements, our framework can quickly obtain the required \textit{N:M} sparse Transformer model with high accuracy, and provide corresponding Transformer accelerators on FPGA devices to realize efficient model deployment.
In this section, we elaborate on the workflow of our algorithm-hardware co-optimized framework.

% [TODO] Overview 的部分应该围绕着图来进行说明。
% At the algorithm level, we mainly focus on how to generate a high inference accuracy but low computational complexity \textit{N:M} sparse Transformer model from a dense one, and how to pack the sparse model into a much slimmer one for memory reduction.
% To this end, we propose an \textit{N:M} incremental dynamic pruning (IDP) method to obtain a 
% At the algorithm level, we focus on how to quickly obtain any desired \textit{N:M} sparse Transformer model, and how to achieve effective compression of the \textit{N:M} sparse Transformer.
At the algorithm level, we focus on quickly obtaining any desired \textit{N:M} sparse Transformer model, and achieving effective compression of the \textit{N:M} sparse Transformer.
The algorithm optimization is divided into two stages.
As shown in Fig.~\ref{fig:workflow}, the first stage is IDP based on the sparsity inheritance mechanism.
% The initial training starts with a dense Transformer to generate the \textit{N:M} sparse parameters of the model, as a model candidate, by updating the mask that indicates the position of the non-zero elements.
% After this round of training, the obtained \textit{N:M} sparse Transformer is added to the candidate pool.
% Then we adjust the parameter \textit{N} for a higher sparsity ratio and start the next round of training.
% The next round of training starts with the recently added candidate model, rather than the dense model, to obtain another \textit{N:M} sparse Transformer candidate with a higher sparsity ratio.
Compared with single-shot training \cite{mishra2021accelerating, zhou2021learning}, our method can utilize the knowledge of the previous \textit{N:M} sparse model, which contributes to faster and better convergence.
% When the pruning stage is over, we select the \textit{N:M} sparse winner model that meets the needs of consumers from the model candidate pool, and pass it to the next stage.
% [TODO] 简单介绍一下 Incremental Dynamic Pruning 的流程，一句话。然后详细的后面再说。
% After several rounds of model accuracy recovery, an \textit{N:M} Transformer model is obtained, which has much lower computational complexity than the dense one.
The second stage is model compression.
Only the non-zero parameters in the \textit{N:M} sparse Transformer would be stored, along with an additional binary mask that indicates position of all recorded elements.
The methods of pruning and model compression are presented in Sec.~\ref{sec:algo}.
% Sec.~\ref{sec:algo} presents the details.

% [TODO] Chao Fang
% \textbf{Q: The workflow of Hardware Auto-generator.}

At the hardware level, we concentrate on efficient and flexible hardware architecture design that boosts the computational efficiency for \textit{N:M} sparse Transformers.
% We further propose an automatic hardware generator based on our architecture to realize agile model deployment for various hardware platforms.
The hardware optimization features an efficient hardware architecture for \textit{N:M} sparse Transformers along with an automatic hardware generator, which can meet requirements on various Transformer models, FPGA devices, and \textit{N:M} sparsity.
The automatic hardware generator is composed of instruction generator and hardware template library.
% The entire hardware workflow are composed of the following components: instruction generator, hardware template library, and \textit{N:M} sparse Transformer accelerator (STA).
% [TODO] 这个部分写的还是太烂了。
% Here we briefly present the workflow of the hardware auto-generator.
% In Sec.~\ref{sec:hwarch}, we elaborate the hardware architecture of STA.
% The generator takes as input the structure of Transformer, hardware parameter configurations, and the \textit{N:M} parameters, and produces as output the optimized STA and instructions that perform operations of the Transformer model.
% When the model is deployed on STA, the compact model parameters and instructions are fed into STA as well.
According to the \textit{N:M} configuration of the winner model and the network structure of the deployment model, the instruction generator can automatically produce instructions that guide STA to perform operations of the winner \textit{N:M} sparse Transformer.
As shown in Fig~\ref{fig:workflow}, instructions are divided into three categories: load/store data, sparse/dense MatMul operators, and fused vector operators.
% Fed with \textit{N:M} configuration and the model structure, the instruction generator would automatically produce instruction flows to perform the operations related to the Transformer.
% The template library accepts the \textit{N:M} configuration and hardware parameters, and automatically generates the corresponding STA.
The hardware template library can quickly generate a dedicated STA based on the pre-defined hardware configurations and the \textit{N:M} configuration of the winner model.
% STA can achieve greatly improvement on computational efficiency when performing inference tasks for Transformers.
STA performs inference tasks for the Transformer model by accessing the compact sparse parameters and the pre-generated instructions.
STA, whose hardware architecture is elaborated in Sec.~\ref{sec:hwarch}, can achieve significant improvement on computational efficiency by eliminating all zero-valued parameter operations.
% The hardware architecture of STA is elaborated in Sec.~\ref{sec:hwarch}.

\RoundOne{
In real-life deployment, the choice of \textit{N:M} may change if there are multiple FPGA devices with different hardware resources, and varying deployment constraints including latency and model accuracy.
% The \textit{N:M} sparsity of Transformers would be a trade-off in terms of model accuracy, inference latency, and hardware cost, as shown in our experimental results on the benchmark set I and II.
% [Chao Fang] 举出一些例子。
% that affect the choice of \textit{N:M}
However, considering all the above factors, once an \textit{N:M} model is determined to be deployed, the model can meet the needs of practical applications.
Therefore, the \textit{N:M} would change before deploying models 
% due to all these factors 
while would not change after the model deployment.
Compared to the Ampere GPU dedicated for \textit{2:4} sparse acceleration, specific \textit{N:M} STA can be flexibly configured and automatically generated on the selected FPGA device with significant performance gains benefited from dedicated \textit{N:M} sparse acceleration.
% , which has performance loss when deploying models with different \textit{N:M} sparsity
% The proposed STA can be generated flexibly when facing various \textit{N:M} configurations and FPGA devices.
As \textit{N:M} changes, our framework would efficiently benefit from the algorithm-hardware co-optimization.
At the algorithm level, the proposed IDP could provide a series of \textit{N:M} models with varying computing complexity and model accuracy, among which we could select the most suitable one for further model deployment.
At the hardware level, the proposed STA could be flexibly generated based on the selected \textit{N:M} and other configurations, achieving significant acceleration of \textit{N:M} Transformers.
}
% \RoundOne{
% For real-life deployment, the choice of \textit{N:M} may change if there are multiple FPGA devices with different hardware resources, multiple deployment constraints including latency and model accuracy. 
% The \textit{N:M} sparsity of Transformers would be a trade-off in terms of model accuracy, inference latency, and hardware cost.
% % that affect the choice of \textit{N:M}
% However, considering all the above factors, once an \textit{N:M} model is determined to be deployed, 
% % we believe that 
% the model can meet the needs of practical applications. Therefore, the \textit{N:M} will change before deploying models while won’t change after the model deployment. Compared to the Ampere GPU, which is merely in favor of \textit{2:4} sparse acceleration, specific \textit{N:M} STA can be flexibly configured and automatically generated on the selected FPGA device with significant performance improvement. 
% The proposed STA can be generated flexibly when facing various \textit{N:M} sparsity and FPGA devices. 
% As \textit{N:M} changes, our framework would efficiently benefit from the algorithm-hardware co-optimization. 
% At the algorithm level, the proposed IDP could provide a series of \textit{N:M} models varying computing complexity and model accuracy, among which we could select the most suitable one for further model deployment. 
% At the hardware level, the proposed STA could be flexibly generated based on the selected \textit{N:M} sparsity and other configurations, achieving significant acceleration of \textit{N:M} Transformers.
% }

==> src/4-sec-algo.tex <==

% \section{获得 \textit{N:M} 稀疏度注意力机制的剪枝算法}


\section{Algorithm Optimization} \label{sec:algo}

In this section, we elaborated on algorithm optimizations of our framework.
% At first, we present the strength of \textit{N:M} sparsity pattern by comparing it with other popular sparsity patterns. 
Firstly, we demonstrate advantages of \textit{N:M} sparsity pattern in Sec.~\ref{subsec:pattern} by comparing it with other popular sparsity patterns. 
Then, pruning algorithm and compression scheme of \textit{N:M} sparse Transformers are presented in Sec.~\ref{subsec:pruning} and Sec.~\ref{subsec:packing}, respectively.

% \begin{itemize}
% 	\item %剪枝问题数学定义。可以直接参考 ICLR'21 文章的定义。
% 	\item %现有的剪枝方法对比。可以跟 arXiv'21 NVIDIA、ICLR'21 的方法进行对比。直接借鉴 arXiv'21 的剪枝图像。
% 	\item %提出自己的剪枝方案。渐进式的 SR-STE finetune 方法。提供具体的算法流程。然后进行文字描述。
% 	\item %基于剪枝方案，继续分析如何由剪枝模型生成硬件可识别的文件。接下来是压缩率理论分析部分。如何进行打包，如何识别。
% \end{itemize}

% \textbf{Q: Why \textit{N:M} sparsity pattern?}

\subsection{\textit{N:M} Sparsity Pattern} \label{subsec:pattern}
% [Q] 这段文字真的有必要加上吗？到底需要多精简的文字？
% Fig.~\ref{fig:pruning_pattern} presents an example of multiple pruning patterns for sparse parameter matrix. 
% Table~\ref{tab:sparsity} presents an example of multiple pruning patterns for sparse parameter matrix. 
%, and a summary of their characteristics.
A dense parameter matrix, can be pruned with a sparsity ratio of 50\% using three existing sparsity patterns, unstructured sparsity \cite{park2020optimus
% , han2015deep, han2015learning
}, block-based structured sparsity \cite{peng2021accelerating
% , narang2017block, varma2019dynamic
}, and \textit{N:M} group-based structured sparsity \cite{zhou2021learning
% ,yao2019balanced,mishra2021accelerating
}, respectively.
Table~\ref{tab:sparsity} summarizes all these pruning patterns.
% Fig.~\ref{fig:pruning_pattern}~(d) summarizes all these pruning patterns.
Elements in any position of the parameter matrix can be pruned if the unstructured sparsity pattern is employed.
% [TODO] 这句话可能也有问题，这里提压缩率很高不太好，因为表格的比较是基于相同的压缩率来对比的。
The unstructured sparse model can achieve a considerable compression ratio while maintaining comparable accuracy to the dense model.
However, there is a limited speedup of the unstructured sparse model on hardware \cite{park2020optimus,tambe2021edgebert} due to the irregular pattern.
% [TODO] 这句话有问题，什么是 unimportant blocks。
For block-based pruning, the parameter matrix is firstly divided into multiple blocks, and then some unimportant blocks was dropped to reduce storage and computing.
% The parameter matrix is firstly divided into multiple blocks, and then pruned 
The block-based sparse model having regular pattern can achieve high computational efficiency on hardware.
% Nevertheless, there is limited compression ratio of the block-based sparse model since the coarse-grained block-based pattern noticeably degrades model accuracy.
Nevertheless, the speedup of block-based sparse models \cite{peng2021accelerating} is inefficient since there is limited compression ratio using the block-based pattern.
As for \textit{N:M} group-based structured sparsity, the parameter matrix is divided into multiple groups.
Here we consider consecutive column-wise elements in the matrix gather as a group.
Each group has \textit{M} elements and contains \textit{N} nonzero elements at most.
The \textit{N:M} sparsity can achieve high compression ratio along with computational efficiency on hardware due to its fined-grained regular pattern.
% [TODO] 这句话想表达两个意思：\textit{N:M} pattern
Hence, Transformers with \textit{N:M} sparsity pattern, which remains a lot to be explored, have much more speedup potential than that with unstructured and block-based sparsity.
% In this section, we exploit how to obtain and pack an optimized \textit{N:M} sparse Transformer from the dense one for saving on storage and computing with negligible loss on model accuracy.
% Among all three sparsity patterns, unstructured sparsity can achieve a considerable compression ratios while maintaining comparable accuracy to the dense model.
% In this example, 
% The dense parameter matrix, as shown in Fig.~\ref{fig:pruning_pattern}(a), can be

%\begin{figure} [htbp] 
%	\centering
%	\includegraphics[width=0.42\textwidth]{figs/TVLSI-4-algo-pruning_pattern-complicated.pdf}
%	\caption{Comparison of three pruning patterns: unstructured sparsity, block-based structured sparsity, and \textit{N:M} group-based structured sparsity.} 
%	\label{fig:pruning_pattern}
%\end{figure}


% \begin{figure}
% \centering
% %\includegraphics[scale=•]{•}egraphics[width=2cm]{examplefigure}
% %\includegraphics[width=2cm]{examplefigure}
% %\includegraphics[width=2cm]{examplefigure}
% %\caption{Example figure caption (floating)}
% %\label{fig:examplefl}

% \begin{tabular}{lccc}
% \hline
% & Accuracy & Efficiency & Speedup\\
% \hline
% Unstructed & High \\
% Block & Low \\
% \hline
% \textbf{N:M} & \textbf{High} & \textbf{High} & \textbf{High} \\
% \hline
% \end{tabular}
% %\captionof{table}{Example Table (floating)}
% \label{tab:examplefl}
% \end{figure} 

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[htbp]
% \centering
% \caption{Summary of existing sparsity patterns}
% \label{tab:sparsity}
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{@{}c|ccc@{}}
% \toprule
%               & Unstructured & Block-based & \textbf{N:M Group-based} \\ \midrule
% Visualization & 

%     \begin{minipage}[b]{0.3\columnwidth}
% 		\centering
% 		\raisebox{-.5\height}{\includegraphics[width=0.6\linewidth]{figs/TVLSI-4-algo-unstructured_pattern.png}}
% 	\end{minipage}
%           &
%     \begin{minipage}[b]{0.3\columnwidth}
% 		\centering
% 		\raisebox{-.5\height}{\includegraphics[width=0.6\linewidth]{figs/TVLSI-4-algo-block_pattern.png}}
% 	\end{minipage}  
%           & 
%     \begin{minipage}[b]{0.3\columnwidth}
% 		\centering
% 		\raisebox{-.5\height}{\includegraphics[width=0.6\linewidth]{figs/TVLSI-4-algo-NM_pattern.png}}
% 	\end{minipage} 
% 	       \\
% Accuracy      & High ↑       & Medium −    & \textbf{High ↑}          \\
% Efficiency    & Low ↓        & High ↑      & \textbf{High ↑}          \\
% Speedup       & Medium −     & High ↑      & \textbf{High ↑}          \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[hbtp]
\centering
\caption{Comparison between existing three sparsity patterns}
\label{tab:sparsity}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{@{}c|ccc@{}}
\toprule
              & Unstructured & Block-based & \textbf{N:M Group-based} \\ \midrule
Visualization &  
    \begin{minipage}[b]{0.3\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=0.6\linewidth]{figs/TVLSI-4-algo-unstructured_pattern.pdf}}
	\end{minipage}
	          &
	 \begin{minipage}[b]{0.3\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=0.6\linewidth]{figs/TVLSI-4-algo-block_pattern.pdf}}
	\end{minipage}  
	          & 
    \begin{minipage}[b]{0.3\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=0.6\linewidth]{figs/TVLSI-4-algo-NM_pattern.pdf}}
	\end{minipage} 
	\\ \midrule
Accuracy      & \textbf{High \checkmark}       & Medium      & \textbf{High \checkmark}          \\ \midrule
Efficiency    & Low        & \textbf{High \checkmark}      & \textbf{High \checkmark}          \\ \midrule
Speedup       & Medium       & \textbf{High \checkmark}      & \textbf{High \checkmark}          \\ \bottomrule
\end{tabular}%
}
\end{table}

% \subsection{Problem Definition}
\subsection{Pruning Algorithm} \label{subsec:pruning}

% \subsubsection{Problem Definition}
Given a pretrained dense Transformer model, generally, a \textit{N:M} sparse Transformer can be trained with the objective as 
\begin{equation}
	\label{equ:def}
	\min_{S(\mathcal{W}, N, M)} \mathcal{L}(\mathcal{W}; \mathcal{D}),
\end{equation}
where $\mathcal{D}$ denotes the observed data, $\mathcal{L}$ represents the loss funtion, $\mathcal{W}$ indicates the parameters of the Transformer, and $S(\mathcal{W}, N, M)$ is the sparse Transformer with \textit{N:M} sparsity pattern. 
% \AJ{
$N$ is the number of non-zero values. For dense model $\mathcal{W}$, it can be equivalent to $S(\mathcal{W},  N=M, M)$.
% }

% \AJ{
Existing methods NVIDIA ASP\cite{mishra2021accelerating} and SR-STE \cite{zhou2021learning} leverage the single-shot magnitude-based pruning and dynamic sparse training from dense models $\mathcal{W}$ respectively. 
The specific sparse models $S(\mathcal{W}, N, M)$ inherit from global dense models $S(\mathcal{W},  M, M)$ with pre-trained weights and random initialization in ASP and SR-STE. 
% The inheritance mechanism ($S(\mathcal{W},  N, M) \leftarrow S(W, M, M)$) 
This may lead to suboptmial problems, and we observe the ASP and SR-STE hurt the performance significantly on Transformer-based models with the higher sparse ratio (e.g., $\geq$75\%). 
In addition, the ASP and SR-STE undesirably require intensive training computation if we have different hardware constraints with multiple sparsity levels (e.g., \textit{1:8}, \textit{2:8}, \textit{3:8} and \textit{4:8}).
% }

% \AJ{
Therefore, we propose a general and simple algorithm for generating models with general \textit{N:M} sparse patterns, namely IDP, which can produce a series of sparse models with different \textit{N:M} configurations. 
Algorithm~\ref{alg:idp} presents the detail of IDP.
To handle the optimization difficulty of the sparse sub-networks inherited from large dense models, we introduce a novel co-training scheme, which optimize different multiple-level \textit{N:M} sparse models simultaneously (e.g., \textit{1:8}, \textit{2:8}, \textit{3:8}, \textit{4:8} and \textit{5:8}). 
During the training phase, we gradually reduce the non-zeros parameters \textit{N}, which can guarantee the super models converge well. We can give the general inheritance mechanism of the IDP as follows:
% }
% \begin{small}
\begin{equation}
    \small
	\label{equ:inherit}
	S(\mathcal{W}, N_1, M) \leftarrow  S(\mathcal{W}, N_2, M) \leftarrow \cdots \leftarrow S(\mathcal{W}, M, M),
\end{equation}
% \end{small}
% \AJ{
where $S(\mathcal{W}, N_i, M)$ are \textit{N:M} sparse models, and the $S(\mathcal{W}, M, M)$ represents the dense model, where $ N_1 < N_2 < \cdots < M $, $\leftarrow$ means the smaller model $S(\mathcal{W},  N-1, M)$ prune from $S(\mathcal{W}, N, M)$, named \textbf{inheritance mechanism}.
It requires merely a hyper-parameter $n$ denoted as the end of iterations of $N$.
% It requires merely a hyper-parameter $n$ denoted as the terminal of iterations of $N$.
% }
% \AJ{
\RoundOne{
With the novel inheritance mechanism, our IDP training method can be summarized with four steps: 
\begin{itemize}
    \item \underline{Step 1:} Initialize $N=M-1$ and set the dense pretrained model as the first winner model.
    \item \underline{Step 2:} Sparsity inheritance applies the kept parameters of the winner of all the $S(\mathcal{W}, N+1, M)$ candidates to initialize following sparse model $S(\mathcal{W}, N, M)$. 
    % \item \underline{Step 2:} Prune and fine-tune an $N=M-1$ sparse model from the dense pretrained model.  
    \item \underline{Step 3:} Sparse training for \textit{N:M} sparse candidates in several epochs. Parameters are adjusted in every epoch by updating the mask based on the their magnitude. This step generates a new winner model, which is the convergent model at the last epoch.
    % \item \underline{Step 3:} Sparsity inheritance, using the kept parameters of $S(\mathcal{W}, N, M)$ to initialize following sparse model $S(\mathcal{W},  N-1, M)$. If $N =n$, the whole process is finished.
% , where $n$ is a hyper-parameter denoted as the terminal . 
    \item \underline{Step 4:} If $N=n$, the whole process is finished, or otherwise $N \leftarrow N-1$, and then go to \underline{Step 2}.
\end{itemize}
}

\RoundOne{
We expect to obtain \textit{M-N+1} preserved winner models with different \textit{N:M} sparsity for subsequent deployment.
Additionally, in the forward pass, we leverage the popular group-wise magnitude pruning \cite{mishra2021accelerating,zhou2021learning}.
Parameter matrices are partitioned into multiple groups, every one of which contains $M$ consecutive column-wise elements, as shown in Table~\ref{tab:sparsity}.
And we keep the $N$-largest parameters in these groups and generate corresponding masks $\mathcal{B} \in \{0,1\}^d$.  Specifically, if the $i$-th parameter of $\mathcal{W}$
survived 
% (not pruned) 
in the pruned sub-network, we set $\mathcal{B}_i = 1$, or else $\mathcal{B}_i = 0$.
% which prune $M-N$ lowest-magnitude weights in each group. 
In the backward pass, recent studies \cite{zhou2021learning,lin2020dynamic} demonstrate that the dynamic sparse training can benefit both model convergence and accuracy, and we follow their methods to calculate gradients. 
}
% We exploit latest dynamic sparse training method SR-STE \cite{zhou2021learning} to recover the accuracy as the following: 
% \begin{align}
%  \mathcal{W}_{t+1} =  \mathcal{W}_t - \gamma_t g( \mathcal{W}_t \odot \mathcal{B}_t) + \lambda((1-\mathcal{B}_t)\odot W_t),
%  \label{scheme:ours}
% \end{align}
% where $\mathcal{B}_t$ denotes the mask for the pruned parameters, $\odot$ denotes Hadamard product, $\lambda$ denotes the relative weight for the sparse-refined term, and $\gamma_{t}$ denotes the learning rate at iteration $t$.

% }
% There are two existing methods to train sparse \textit{N:M} networks: NVIDIA ASP \cite{mishra2021accelerating} and SR-STE \cite{zhou2021learning}.
% % As shown in Fig.~\ref{fig:pruning_method}(a), ASP only prunes the model once at the beginning of accessing the pre-trained model.
% % The model connection achieving the target sparsity is frozen in the ASP pruning step.
% As shown in Fig.~\ref{fig:pruning_method}~(a), ASP leverages the single-shot magnitude-based pruning to obtain the 2:4 sparsity from pre-trained dense models.
% SR-STE, as presented in Fig.~\ref{fig:pruning_method}~(b), trains a model from scratch with a dynamic \textit{N:M} mask, using a sparse-refined straight-through estimator (SR-STE), but results for 2:4 sparsity fall short of the dense baseline.
% We observe the ASP and SR-STE hurt the performance significantly on transformer-based models with the higher sparse ratio (e.g., $\geq$75\%).
% To facilitate arbitrary \textit{N:M} sparse neural networks deployment on FPGA, we propose a general and simple algorithm for arbitrary \textit{N:M} sparse pattern, named Inherited Dynamic Pruning (IDP). \AJ{xxx, In this paper, }

\begin{algorithm}
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{Inherited Dynamic Pruning}
	\label{alg:idp}
	\begin{algorithmic}[1]
	    \REQUIRE Pre-trained dense weights $\mathcal{W}$, datasets $\mathcal{D}$, initial learning rate $\gamma_{0}$ and the end of iterations $n$.
        \FOR{$N=M-1, M-2,.., n$}
        %   \STATE sparse inher
           \STATE \RoundOne{\textbf{Sparsity Inheritance}: \\ ~~$S(\mathcal{W}, N, M) \leftarrow$ the winner of $S(\mathcal{W}, N+1, M)$.}
           \FOR{each training iteration $t$}
             \STATE \textbf{Forward Pass}: 
                \\ ~~generate $\mathcal{B}_t$ by group-wise magnitude pruning.
             \STATE \textbf{Backward Pass}: 
                \\ ~~$\mathcal{W}_{t+1} =  \mathcal{W}_t - \gamma_t g( \mathcal{W}_t \odot \mathcal{B}_t) + \lambda((1-\mathcal{B}_t)\odot W_t)$.
            %  \STATE Update $S(\mathcal{W}, N, M)$.
           \ENDFOR
        %   \STATE \RoundOne{Winner Generation: The convergent $S(\mathcal{W}, N, M)$ candidate in the final iteration. }
        \ENDFOR
	    \ENSURE \RoundOne{A series of \textit{N:M} sparse models with different computation complexity and corresponding masks: the winners of $S(\mathcal{W},  N=M-1, M)$, $S(\mathcal{W},  N=M-2, M)$,.., $S(\mathcal{W},  N=n, M)$.}
	    %\STATE \textbf{return} $\widetilde{\mathcal{W}}, \bar{\varepsilon}$
	\end{algorithmic} 
\end{algorithm} 

%In algorithm, we using the popular magnitude pruning during, which prune 

% Algorithm \ref{alg:idp} presents the detail of IDP.

% \begin{algorithm}
% 	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
% 	\renewcommand{\algorithmicensure}{\textbf{Output:}}
% 	\caption{Inherited Dynamic Pruning}
% 	\label{alg:idp}
% 	\begin{algorithmic}[1]
% 	    \REQUIRE Pre-trained dense weights $\mathcal{W}$, datasets $\mathcal{D}$, initial learning rate $\gamma_{0}$, 
% 	    group size $M$, model performance $y_{0}$ and acceptable performance drop $\delta$.
% 	    \ENSURE The \textit{N:M} sparse weights $\widetilde{\mathcal{W}}$, and corresponding bitmasks $\bar{\varepsilon}$.
% 	   % \STATE \textbf{Input:} Pre-trained dense weights 
% 	    \STATE Initialize $N \leftarrow M, \widetilde{\mathcal{W}} \leftarrow \mathcal{W}, \bar{\varepsilon} \leftarrow $ \textbf{ones}$(\mathcal{W})$
% 	    \WHILE{$N > 1$}
% 	        \STATE $N \leftarrow N-1$, $\gamma \leftarrow \gamma_{0}$
% 	        \FOR{each training epoch $p$}
%         	    \FOR{each training iteration $t$}
%         	        \STATE Sampling a batch $b_{t} \sim \mathcal{D}_{train}$
%         	        \STATE $\bar{\varepsilon}_{t} \leftarrow $ \textbf{MaskUpdate}$(\mathcal{W}, N, M)$
%         	        \STATE $\widetilde{\mathcal{W}}_{t} \leftarrow  \mathcal{W} \odot \bar{\varepsilon}_{t}$
%         	        \STATE $y_{t} \leftarrow $ \textbf{ForwardPass}$(\widetilde{\mathcal{W}}_{t}, b_{t})$
%         	        \STATE $\mathcal{W}, \gamma \leftarrow$ \textbf{BackwardPass}$(\mathcal{W}, \bar{\varepsilon}_{t}, b_{t}, \gamma, \mathcal{L}(y_{t}; b_{t}))$
%         	    \ENDFOR
%         	    \STATE $\bar{\varepsilon}_{p} \leftarrow $ \textbf{MaskUpdate}$(\mathcal{W}, N, M)$
%         	    \STATE $\widetilde{\mathcal{W}}_{p} \leftarrow  \mathcal{W} \odot \bar{\varepsilon}_{p}$
%         	    \STATE $y_{p} \leftarrow $
%         	    \textbf{PerformanceEvaluation}$(\widetilde{\mathcal{W}}_{p}, \mathcal{D}_{eval})$
%         	    \IF{$\delta > y_{0} - y_{p}$}
%         	        \STATE \textbf{return} $\widetilde{\mathcal{W}}, \bar{\varepsilon}$
%         	    \ENDIF
%         	    \STATE $\widetilde{\mathcal{W}} \leftarrow \widetilde{\mathcal{W}}_{p}, \bar{\varepsilon} \leftarrow \bar{\varepsilon}_{p}$
%             \ENDFOR
%             % \STATE \textbf{return} $\widetilde{\mathcal{W}}, \bar{\varepsilon}$
% 	    \ENDWHILE 
% 	    \STATE \textbf{return} $\widetilde{\mathcal{W}}, \bar{\varepsilon}$
% 	\end{algorithmic} 
% \end{algorithm} 

% \textbf{MaskUpdate.} It consists of three steps: Firstly, group elements. For a given parameter matrix, we partition it into multiple groups, every one of which contains $M$ consecutive column-wise elements, as shown in Fig.~\ref{fig:pruning_pattern}~(c). 
% Secondly, preserve parameters. 
% We sort the elements for each groups in parallel, keep the $N$-largest parameters, and set others as zero. 
% Here, we adopt the sorting metric based on the value magnitude. 
% Finally, generate masks. 
% We identify a mask for each group to label positions of non-zero parameters, and then, merge all these masks into a matrix, $\bar{\varepsilon}$. 

% \textbf{ForwardPass.} Unlike the general workflow, we here utilize the \textit{N:M} sparse parameters for forward propagation. 
% % [Note] Chao Fang: 这里可以补充一下这么做的原因。
% The sparse matrix of parameters could be easily generated by element-wise multiplying dense parameters with the mask matrix.

% \textbf{BackwardPass.} It contains two steps: backward propagation, and weight update.
% In backward propagation, the gradients related to parameters are originated from the forward pass with the sparse parameters.
% Note that all parameters, including those being pruned in the forward pass, are backward propagated and updated in the backward pass.
% We introduce the sparse-refined term in \cite{zhou2021learning} to penalize the parameters being pruned in $\widetilde{\mathcal{W}}$ and decrease the magnitude of the these parameters. 
% The rule of weight update is presented in \ref{equ:refined_term_SRSTE}, where $\bar{\varepsilon}$ denotes the mask for the pruned weights, $\odot$ denotes Hadamard product, $\lambda$ denotes the relative weight for the sparse-refined term, and $\gamma_{t}$ denotes the learning rate at iteration $t$.

% \begin{equation}
% 	\label{equ:refined_term_SRSTE}
% 	\mathcal{W}_{t+1} = \mathcal{W}_{t} - \gamma_{t}(g(\widetilde{\mathcal{W}}_{t})+ \lambda ( \bar{\varepsilon}_{t} \odot \mathcal{W}_{t}) ),
% \end{equation}

% \begin{figure*} [htbp] 
% 	\centering
% 	\includegraphics[width=0.86\textwidth]{figs/TVLSI-4-algo-pruning_method.pdf}
% 	\caption{Illustrations of training stages between (a) ASP \cite{mishra2021accelerating}, (b) SR-STE \cite{zhou2021learning} and (c) our proposed IDP to obtain a $2$:$4$ sparse Transformers.} 
% 	\label{fig:pruning_method}
% \end{figure*}

% \AJ{SR-STE proposes to train a model from scratch with a dynamic \textit{N:M} mask, using a sparse-refined straight-through estimator (SR-STE), but results for 2:4 sparsity fall short of the dense baseline.}
% [TODO] 这段话也需要重写，太差了。


% ASP:

% \begin{equation}
% 	\label{equ:refined_term_ASP}
% 	\widetilde{\mathcal{W}}_{t+1} = \widetilde{\mathcal{W}}_{t} - \gamma_{t} g(\widetilde{\mathcal{W}}_{t}),
% \end{equation}

% SR-STE \textbf{TODO}

% \begin{equation}
% 	\label{equ:refined_term_SRSTE}
% 	\mathcal{W}_{t+1} = \mathcal{W}_{t} - \gamma_{t}(g(\widetilde{\mathcal{W}}_{t})+ \lambda ( \bar{\varepsilon}_{t} \odot \mathcal{W}_{t}) ),
% \end{equation}

% \AJ{ASP leverages the single-shot magnitude-based pruning to obtain the 2:4 sparsity from pre-trained dense models. We observe the ASP and SR-STE hurt the performance significantly on transformer-based models with the higher sparse ratio (e.g., $\geq$75\%), To facilitate arbitrary \textit{N:M} sparse neural networks deployment on xxx, we propose a general and simple algorithm for arbitrary \textit{N:M} sparse pattern, named (IDP), }

% % [TODO] 这是写算法好，还是写流程好？
% \begin{figure} [htbp] 
% 	\centering
% 	\includegraphics[width=0.46\textwidth]{figs/TVLSI-4-algo-pruning_flow.pdf}
% 	\caption{The flow chart of IDP.} 
% 	\label{fig:pruning_flow}
% \end{figure}




\begin{figure} [htbp] 
	\centering
	\includegraphics[width=0.42\textwidth]{figs/TVLSI-4-algo-compressed_storage.pdf}
	\caption{Compact storage scheme example for \textit{N:M} sparse parameter matrix.} 
	% \caption{Compact storage scheme for $2$:$4$ sparse parameter matrix.} 
	\label{fig:compressed_format}
\end{figure}

\subsection{Packing \textit{N:M} Sparse Parameters} \label{subsec:packing}

An \textit{N:M} sparse Transformer can be obtained after IDP, where each group of all parameter matrices only contains at most $N$ non-zero elements.
However, it occupies a large amount of memory since the parameter store scheme is the same as the dense Transformer.
% We propose a method to obtain a compact \textit{N:M} sparse Transformer, which greatly achieves saving on storage and computing for deployment.
\RoundOne{
We apply the bitmap-based compression scheme to obtain a compact \textit{N:M} sparse Transformer, which greatly achieves saving on storage for deployment.
Compared to COO, CSC, CSR \cite{hoefler2021sparsity}, and step indexing \cite{zhang2016cambricon}, our scheme has better compression performance in the range of practical \textit{N:M} sparsity.}
Fig.~\ref{fig:compressed_format} presents the compression scheme of \textit{N:M} sparse parameter matrix using \textit{2:4} sparsity as an example.
For a parameter matrix $W\in\mathbb{R}^{R\times C}$, after IDP, there are at most \textit{2} non-zero elements in a group.
The entire parameter matrix has $\frac{R}{2} \times C$ remaining non-zero elements.
In our scheme, we merely preserve non-zero elements in each group, and use a binary mask to indicate the elements' position.
By using our scheme, a \textit{2:4} parameter matrix $W\in\mathbb{R}^{R\times C}$ can be stored with $\frac{R}{2} \times C$ valid elements and $R \times C$ bits for the mask, instead of the $R \times C$ elements.

Considering a dense parameter matrix $W\in\mathbb{R}^{R\times C}$, in which all elements are quantized using $q$ bits.
% Followed by our continuous \textit{N:M} pruning, 
% matrix 
$W$ can be compressed to $\tilde{W}\in\mathbb{R}^{R \times \lceil \frac{C}{M} \rceil N}$, where there are $R\lceil \frac{C}{M} \rceil$ groups and each group has $N$ non-zero parameters at most.
The storage requirement of $W$ is $qRC$ bits, and after pruning, we can only store the \textit{N:M} sparse matrix $\tilde{W}$ in a compact way with only  $qR\lceil\frac{C}{M}\rceil N$ bits, and an additional binary mask with $RC$ bits.
Therefore, the compression ratio (CR) can be represented as: 

\begin{equation}
	CR = \frac{qC}{q\lceil\frac{C}{M}\rceil N+C}.
	\label{equ:compression_ratio}
\end{equation}

==> src/5-sec-hwaccel.tex <==

\section{Hardware Optimization} \label{sec:hwarch}

% \begin{itemize}
% 	\item % 硬件整体概述。是基于模板进行生成的。整个加速器是如何进行运作的。
% 	\item % 计算阵列设计。
% 	\item % 计算PE设计。包括 \textit{N:M} 多路选择器，以及乘加器的设计。
% 	\item % Softmax 硬件单元的设计。
% 	\item % LayerNorm 硬件单元的设计。
% \end{itemize}

The flexible and efficient hardware architecture, namely STA, is developed for \textit{N:M} sparse Transformers in this section.
We first present the overall architecture of STA, and then elaborate on designs of its core computing engines, including DMME and scalable softmax module.

\begin{figure} [hbtp] 
	\centering
	\includegraphics[width=0.46\textwidth]{figs/TVLSI-5-hwaccel-arch.pdf}
	\caption{The overall architecture of STA. It is composed of computing, storage, and control function blocks. These red arrows pass control signals, while those black arrows transfer data.} 
	\label{fig:arch}
\end{figure}

\subsection{Overall Architecture} \label{subsec:ova}
The overall architecture of STA is shown in Fig.~\ref{fig:arch}, which consists of three major function blocks, including computing, storage, and control. 
The computing blocks consist of a diverse MatMul computing engine , namely DMME, a scalable softmax module, a vector unit, and a data reshuffle network.
% [TODO] Chao Fang: 这里是否要突出一下性能呢？还是普通叙事功能呢？
Dominated operations of \textit{N:M} sparse Transformers, i.e. sparse-dense or dense-dense MatMuls, are performed by DMME on-the-fly with the dynamic configuration under high computational efficiency.
The scalable softmax module is responsible for the softmax operation in MHA ResBlocks, eliminating the off-chip transfer for intermediate data.
The vector unit takes charge of operations with low computational density including bias addition, residual addition, and activation functions.
The reshuffle network reorders the temporary results before writing back to the intermediate on-chip memory.
% [TODO] Chao Fang: 讲一下 storage design consideration
% [TODO] Chao Fang: 太难写了这里，插一个断点，后面有思路了再回来写
% Benefitting from the group-based pruning scheme, 
As for on-chip storage, it can be partitioned into three parts, including the weight memory, the input memory, and the intermediate memory. 
The weight and input memory store model parameters and input data of Transformers from the off-chip memory, respectively.
The results of a ResBlock are also written back to the input memory, and pass to the off-chip memory.
And all the temporary results in a ResBlock will be stored in the intermediate memory with no communication to the external memory.
% [TODO] Chao Fang: 这里是不是需要提一下每个Mem的Access情况？比如说，是否乒乓Buffer？Weight Memory 是双向的，Input Memory 是单向的。Intermediate Memory是不与外部Memory通信的。


\begin{figure} [hbtp] 
	\centering
	\includegraphics[width=0.48\textwidth]{figs/TVLSI-5-hwaccel-dmme_microarch.pdf}
	\caption{The hierarchical architecture of DMME. It consists of $H$ parallel unified MatMul computing engine (a). Each engine contains $R \times C$ unified systolic PE capable of handling both sparse-dense and dense-dense dot products (b). The key components of PEs, non-zero element selector and the \textit{N}-parallel MAC, are in (c) and (d), respectively.} 
	\label{fig:mircoarch}
\end{figure}

\subsection{DMME} \label{subsec:DMME}
DMME unifies both sparse-dense and dense-dense MatMuls with a high computational efficiency in \textit{N:M} sparse Transformers. 
When it performs sparse-dense MatMuls, it merely loads nonzero weight parameters and selects corresponding activations to compute, thereby improving computational efficiency. 
% As for dense-dense MatMuls, it efficiently acts the same as the systolic array in \cite{lu2020hardware}. 

The architecture of the DMME is illustrated in Fig.~\ref{fig:mircoarch}. 
It is a two-level hierarchy design with a full exploration of parallelism inside the MatMuls of \textit{N:M} sparse Transformers.
The exploited parallelism consists of head parallelism, row parallelism, and column parallelism, which are denoted as $H$, $R$, and $C$, respesctively.
The DMME is composed of $H$ parallel $R\times C$ unified MatMul computing engine (Fig.~\ref{fig:mircoarch}~(a)), every one of which can efficiently realize both sparse-dense and dense-dense MatMuls in a time-division multiplexing manner.
The capability of performing sparse-dense and dense-dense MatMuls comes from the inner unified systolic PE (Fig.~\ref{fig:mircoarch}~(b)).
It is composed of a non-zero element selector, a \textit{N}-parallel MAC, multiple multiplexers, and registers.
The non-zero element selector, only being activated in the sparse-dense MatMul mode, is to select the proper activation according to the input bitmask.
% [Note] Chao Fang: ~~下面的 N-par MAC 写的不够抽象，功能没有描述清楚。~~
The \textit{N}-parallel MAC accepts \textit{N} \textit{16}-bit input data and parameters, realizes inner product, and then accumulates the result with the local \textit{32}-bit output partial sum.
The multiplexers and registers are used for datapath selection and temporary data storage, respectively.
% [TODO] Chao Fang: 后面几段需要详细考虑。
% The non-zero element selector takes as input a $M$-bit mask, where the mask merely contains \textit{N} 1 bits to indicate the non-zero element position. 
The design of non-zero element selector is presented in Fig.~\ref{fig:mircoarch}~(c).
It takes as input an \textit{M}-bit mask, in which only \textit{N} bits are set as \textit{1} to indicate the position of non-zero elements, and then generates \textit{N} one-hot encoding masks to select the corresponding \textit{N} data for dot product computation.
% [Q] Chao Fang: 在描述的时候是不是太过于平淡，过于着重设计本身，而突出该设计的优势呢？
The translation to \textit{N} one-hot encoding masks is performed by cascading the simple bit-arithmetic blocks and \textit{XOR} gates.
With the help of \textit{N} one-hot encoding masks, data related to non-zero parameters are fed into the \textit{N}-parallel MAC along with these non-zero parameters in one group.
\RoundOne{It could be pointed out that the non-zero element selector can be further optimized by pruning the redundant indexing indicators and element candidates.}
The \textit{N}-parallel MAC, as shown in Fig.~\ref{fig:mircoarch}~(d), is composed of \textit{N} parallel multipliers, an adder tree, and a final accumulator.
% [Q] Chao Fang: 这里是否需要再多讲讲 N-parallel MAC 呢？
Both non-zero element selector and \textit{N}-parallel MAC are fully pipelined to maximize the throughput of DMME.
% At first, it generates \textit{N} one-hot encoding masks, and selects the corresponding \textit{N} data for further computation

% [Note] Chao Fang: 感觉我写的这部分缺少 Insight: Design Consideration.

\begin{figure} [htbp] 
	\centering
	\includegraphics[width=0.48\textwidth]{figs/TVLSI-5-hwaccel-datapath.pdf}
	\caption{The activated datapath of PEs under (a) dense-dense and (b) sparse-dense modes.} 
	\label{fig:datapath}
\end{figure}

The activated datapath under dense-dense and sparse-dense MatMuls are presented in Fig.~\ref{fig:datapath}~(a) and (b), respectively.
The dense-dense mode of PEs would be only activated when performing the self-attention operation of MHA.
Both input operands are arranged in dense sequences in this mode.
% The operation of dense-dense MatMul is appeared in the self-attention of MHA. 
In this case, \textit{N} elements, as an operand, in the input sequences are in parallel streamed into the PE from the west and the north, respectively.
In a cycle, the PE performs a dot product with a size of \textit{N} under dense-dense mode.
The partial sum is stored in the local registers, and the input operands from the west and the north stored in the registers are passed into adjacent PEs on the east and south, respectively.
% The non-zero element selector is bypassed to save energy.
For energy saving, the non-zero element selector is bypassed to avoid signal switching.
% There is no signal switching in the non-zero element selector since it is bypassed.
% There are \textit{N} elements parallelly streaming into the PE in a cycle.
Under sparse-dense MatMul mode, as shown in Fig.~\ref{fig:datapath}~(b), the input operands is different from that under the dense-dense mode.
In a cycle, \textit{N} non-zero parameters in a group along with the corresponding $M$-bit mask are streamed into the PE from the west, while $M$ data in one group are fed from the north.
The \textit{N} valid data in pair with the input parameters is picked up by the non-zero element selector, and then performs a dot product with these input parameters.
% The local register updates the sum accumulating with the result of the dot product.
% The input operands of the PE from the west and the north, temporally stored in the registers, are passed into the adjacent PEs on the east and the south, respectively.
When the computing task is done, under either dense-dense or sparse-dense modes, the PE turns into the shifting mode, accepts the results from its western PE to its local registers and transfers its local result registers to the east.

\begin{figure} [hbtp] 
	\centering
	\includegraphics[width=0.48\textwidth]{figs/TVLSI-5-hwaccel-dmme_dataflow_simple.pdf}
	\caption{\RoundOne{Computing dataflows of DMME when it performs (a) dense-dense and (c) sparse-dense MatMuls. Compared to (b) as a baseline, (c) eliminates all zero-valued redundant operations under sparse-dense mode, thus improving computational efficiency.}}
	\label{fig:dmme_dataflow}
\end{figure}

\subsection{\RoundOne{Supporting Efficient Matrix Computations}}

\RoundOne{
STA is capable of supporting both sparse-dense and dense-dense MatMuls of \textit{N:M} sparse Transformers in an efficient way.
We demonstrate this significant capability of STA by exploiting four aspects: the computing dataflow of DMME, data access pattern of DMME, data mapping of input memory, and datapath from input memory to DMME.
}

\RoundOne{
% Fig.~\ref{fig:dmme_dataflow} illustrates how the DMME supports both dense-dense and sparse-dense MatMuls in a computation-efficient manner when compared with the classic systolic array \cite{lu2020hardware}.
Fig.~\ref{fig:dmme_dataflow} illustrates efficient computing dataflows of DMME under both dense-dense and sparse-dense modes.
For simplicity, we assume \textit{N:M} is \textit{1:2}, and MatMul is performed by $2 \times 4$ input sequences and $4 \times 2$ parameter sequences.
Here, we consider the computing engine in \cite{lu2020hardware} as a baseline, which is orchestrated as a classic systolic array.
In Fig.~\ref{fig:dmme_dataflow}~(a), DMME finishes the dense-dense MatMul in the given computing task using \textit{5} cycles, which consumes the same cycles as the baseline.
Hence, DMME achieves the same computational efficiency as the baseline when performing dense-dense MatMuls.
As for sparse-dense MatMuls, Fig.~\ref{fig:dmme_dataflow}~(b) and (c) present the computational manner of the baseline and DMME, respectively.
The baseline takes \textit{5} cycles to finish the task, while it cost merely \textit{3} cycles by DMME since the redundant operations can be skipped with no waste on computing cycles.
% when compared with the classic systolic array \cite{lu2020hardware}.
% Under the sparse-dense mode, DMME significantly reduces the computational complexity by performing calculations with non-zero parameters, thereby shortening latency and saving power.
% compared to the computing engine in \cite{lu2020hardware}.
% Under the sparse-dense mode, DMME achieves significant computing reduction by performing calculations with non-zero parameters, thereby shortening latency and saving power compared to the computing engine in \cite{lu2020hardware}.
% It is presented using \textit{N:M} as 1:2 for simplicity.
% In Fig.~\ref{fig:dmme_dataflow}~(a), the unified systolic array performs dense-dense MatMuls with the same computational efficiency as the classic array. 
% Fig.~\ref{fig:dmme_dataflow}~(d) further summarizes the computing dataflows of the baseline and DMME.
For sparse-dense MatMuls, DMME improves the computational efficiency by eliminating redundant computations, thereby significantly reducing latency and energy.
% and thereby achieving significant reductions on execution cycles.
% Nevertheless, the classic systolic fails to skip the redundant pruned computations, 
% There is no redundant computation in DMME when performing sparse-dense MatMul,improving the PE utilization and thereby achieving reductions on execution cycles.
}


\begin{figure} [htbp] 
	\centering
	\includegraphics[width=0.48\textwidth]{figs/TVLSI-5-hwaccel-data_access_pattern.pdf}
	\caption{Data access pattern of DMME to support efficient MatMuls under (a) dense-dense and (b) sparse-dense modes.}
	\label{fig:dmme_pattern}
\end{figure}

\RoundOne{
Fig.~\ref{fig:dmme_pattern}~(a) and (b) presents data access patterns of DMME when it
performs dense-dense and sparse-dense MatMuls, respectively.
For dense-dense MatMuls, attention heads as input are both separated into $H$ tiles.
In this case, DMME can be decomposed as $H$ independent systolic arrays, every one
of which fetches elements from the corresponding tiles to the top-most and left-most PEs, respectively.
For sparse-dense MatMuls, compressed weight parameters are divided into $H$ tiles.
Every cycle DMME fetches $NR$ weight elements from all $H$ tiles in parallel, and casts them one-on-one to the left-most systolic PEs in $H$ systolic arrays. 
DMME is also required to access $MC$ activation elements, and broadcasts them to the top-most PEs in all $H$ unified systolic arrays.
% [Note] Chao Fang: 怎么理解这句话呢
% The number of accessed data could stay the same under both computing modes if we set $NH$ as $M$ in the hardware configuration of STA.
}

\RoundOne{
To balance the bandwidth of input memory when switching between dense-dense and sparse-dense modes, we make $NH$ equal to $M$ of STA.
There are $C$ banks of STA for input data storage.
Fig.~\ref{fig:input_mem} illustrates data mapping of input memory and datapath from input memory to DMME by assuming $N$ is 2, $M$ is 4, $H$ is 2, and $C$ is 4.
The data storage storage structure in the input memory is varied for different computing modes.
In dense-dense mode, DMME performs 2 parallel dense-dense MatMuls for attention mechanism of Transformers. 
There are 2 tiles for the loaded input data. 
As shown in Fig.~\ref{fig:input_mem}~(a), the first bank is connected to the first column of DMME, and the first address of the bank indexes the data from the first 2 elements at the first column in the tile one and two, respectively. 
% In sparse-dense mode, we do not tile input data for sparse-dense MatMul.
In sparse-dense mode, DMME performs MatMuls with the \textit{N:M} sparse parameters. 
As depicted in Fig.~\ref{fig:input_mem}~(b), we do not tile input data for sparse-dense MatMul.
The first address of bank one that connected to the first column of
DMME, indexes the data from the first 4 elements at the first column of input data.
It is the same of the indexing principle for the other banks in both computing modes.
}

\begin{figure} [htbp] 
	\centering
	\includegraphics[width=0.48\textwidth]{figs/r1-TVLSI-4-input_mem_structure.pdf}
	\caption{\RoundOne{Data mapping of input memory and datapath from input memory to DMME under (a) dense-dense and (b) sparse-dense modes.}}
	\label{fig:input_mem}
\end{figure}

\RoundOne{
% As for the datapath from input memory to DMME, we takes the first column of DMME as an example. 
% There are 4 elements accessed from the first bank streaming to the first column with a head dimension of 2. 
% The unified systolic PE in the first head of the first column directly receives these 4 elements. 
% The lowest 2 elements are fed into \textit{N}-parallel MAC for computing, while the masked highest 2 elements have no effect on results. 
% However, the unified systolic PE in the second head of the first column requires 2-to-1 MUXs to select the correct 2 elements for computing.
% In sparse-dense mode, data accessed from the first bank broadcast to unified systolic PEs in all head dimensions of the first column of DMME.
As for the datapath from input memory to DMME, we takes the first column of DMME as an example.
There are 4 elements accessed from the first bank streaming to the first column with a head dimension of 2.
In dense-dense mode, as shown in Fig.~\ref{fig:input_mem}~(a), the unified systolic PE in the first head of the first column directly receives these 4 elements, and the lowest 2 elements are fed into \textit{N}-parallel MAC for computing.
% , while the masked highest 2 ($M-N$) elements have no impact on results.
However, the unified systolic PE in the second head of the first column requires 2-to-1 MUXs to select the correct 2 elements from the 4 accessed elements for computing.
In sparse-dense mode, as presented in Fig.~\ref{fig:input_mem}~(b), data accessed from the first bank broadcast to unified systolic PEs in all head dimensions of the first column of DMME.
}


\subsection{Scalable Softmax Module} \label{subsec:softmax}

% As shown in Equ. \ref{equ::softmax}, we need to implement an efficient exponential function, an accumulator, and a flexible divider when considering how to design an softmax architecture.
% The softmax function is used to maximize the probability distribution over predicted output classes in CNNs. 
% Since it only appears once in the last layer of CNNs, it is unprofitable to implement this function on the chip.
% Nevertheless, the softmax function appears frequently in the inner MHA modules of the Transformer. To reduce the reloading frequency of intermediate results for softmax operators, it is essential to implement a scalable softmax module on the accelerator. 
% It is required to perform the softmax function in each MHA module of Transformers. That is totally different from that in CNNs, since the softmax function only appears once in the last layer of CNNs.
% It is unprofitable for chips dedicated to CNNs to implement the softmax function because it only appears once in the last layer of CNNs.

The softmax function takes as input a vector $\textbf{x}$ of $n$ real numbers, and normalizes it into a probability distribution consisting of $n$ probabilities proportional to the exponentials of the input numbers.
% It is defined by the formula:
% \begin{equation}
% 	softmax(\textbf{x})_{i} = \frac{e^{x_i}}{\sum_{j=1}^{n} e^{x_j}} \quad \text{for } i = 1, ..., n.
% 	\label{equ::softmax}
% \end{equation}
% Transformer accelerators are required to contain a softmax hardware implementation since the softmax function appears in every MHA module of Transformers.
It is critical for Transformer dedicated accelerators to contain a softmax hardware implementation since the softmax function appears in every MHA module of Transformers.
Fig.~\ref{fig:softmax} presents the details of our proposed scalable softmax architecture, which is capable of performing softmax functions of arbitrary length. 
It keeps all the intermediate results fully local, avoiding off-chip data communication.

The architecture has two adjustable parameters, $P$ and $Q$, where $P$ denotes the parallelism of the architecture, and $Q$ represents the pipeline depth, as well as the output precision.
$P$ input data are streamed into the softmax module in parallel, and transformed into the exponent outputs.
The exponent outputs are not only temporarily stored in the data buffer, but also used as input for further accumulation.
% $P$ input data are streamed into the softmax module in parallel, and the exponent outputs are not only performed accumulation using an adder tree, but also temporarily stored in the data buffer. 
Once the accumulation process is done, the divider module takes both accumulated results and exponent outputs as input to perform $Q$-level pipelined division, and generates $P$ softmax function outputs represented by $Q$-bit.

\begin{figure} [hbtp] 
	\centering
	\includegraphics[width=0.48\textwidth]{figs/TVLSI-5-hwaccel-softmax.pdf}
	\caption{The architecture of the scalable softmax operator.} 
	\label{fig:softmax}
\end{figure}

As shown in Fig.~\ref{fig:softmax}, the scalable softmax module consists of three major parts: an area-efficient exponential function, a partial sum accumulator, and a scalable divider.
%We propose a mixed-mode $e^x$ design to shrink the resource utilization of lookup table. 
%At first, the input was cut into two parts. 
% [TODO] 这里说的很啰嗦
%The part containing the most significant bit was set to a lookup table to acquire the result, while the other part is approximated with the $1^{st}$ order Taylor expansion.
% The exponential function is approximated by the method combined with lookup table query and the $1^{st}$ order Taylor expansion.
The exponential function is approximated using a lookup table combined with a first-order Taylor expansion.
An exponential operator can be implemented using only one multiplier and one adder.
The configurable partial sum accumulator can adapt to input vectors of various lengths, which improves the flexibility of the hardware.
% There are $d_k$ times divisions in a softmax function.
% The computational efficiency would be severely affected if the latency of the divider is too long.
% To reduce the latency of the division, we design a highly parallel divider by cascading multiple divider blocks with pipelines.
To reduce the latency of the division, we design a highly parallel divider by cascading multiple divider blocks with pipelines, where a divider block is composed of subtractors and shifters with little cost on hardware.
% The precision of the divider can be adjusted by the pipeline length.
% The fully pipelined softmax architecture can overlap the division of the previous vector and the exponent operation of the current vector. 



==> src/6-sec-res.tex <==
\section{Experimental Results} \label{sec:res}

% 算法上的实验。考虑三类应用以及相应典型模型。主要体现剪枝方案的可行性以及精度比较。
% \begin{itemize}
% 	\item 算法实验选取模型以及数据集。
% 	\begin{itemize}
% 		\item Sequence Classification
% 		\begin{itemize}
% 			\item 模型：BERT-base
% 			\item 数据集：MNLI，MRPC，QNLI，QQP
% 		\end{itemize}
% 		\item Translation
% 		\begin{itemize}
% 			\item 模型：T5-small
% 			\item 数据集：wmt16-ro2en, iwslt17-de2en
% 		\end{itemize}
% 		\item Image Classification
% 		\begin{itemize}
% 			\item 模型：vit-base-patch16-224-in21k。注意，该模型的关键结构与 BERT 是相同的。但是还有一层 MLP。计算量上还是有微小的区别。
% 			\item 数据集：beans, cats\_vs\_dogs
% 		\end{itemize}		
% 	\end{itemize}
% 	\item 不同稀疏度下不同应用不同剪枝方法的剪枝曲线。不同剪枝方法4种对比：随机剪枝、Nvidia的ASP剪枝、SR-STE的一次性剪枝。
% 	\item 相同稀疏度下对不同部分剪枝的影响。不同部分剪枝：只剪注意力模块、只剪前馈神经网络、同时剪注意力模块和前馈神经网络。
% 	\item 不同稀疏度下对不同部分剪枝取得的真实数据压缩比。不同部分剪枝：只剪注意力模块、只剪前馈神经网络、同时剪注意力模块和前馈神经网络。
% \end{itemize}

% \vspace{2ex}

% 硬件上的实验。主要体现硬件方案的灵活性，以及相应的加速效果。灵活性指，可对加速器内的关键组件进行灵活配置，并可部署在不同的板子上。
% \begin{itemize}
% 	\item 不同硬件配置下的矩阵计算模块的资源消耗，以及与仅支持稠密矩阵计算模块的overhead对比。
% 	\item 不同硬件配置下的计算加速比。
% 	\item 选取两块不同的板子，根据资源以及精度进行部署，给出整体的综合结果。
% 	\item 与同期Transformer硬件加速的工作进行对比，列出表格。
% \end{itemize}

In this section, we comprehensively evaluate both algorithm and hardware optimizations of the proposed framework.
Three benchmark sets with varying size and complexity are applied to evaluate the proposed framework.

\subsection{Experimental Setup}

\subsubsection{\textbf{Benchmark Sets}}
~
\newline
\indent The first set focuses on the evaluation of algorithm optimizations, by comprehensively presenting improvements on both model accuracy and compression ratio under various \textit{N:M} configurations.
This benchmark set comprises a BERT model \cite{kenton2019bert}, the well-known Transformer-based model, and four evaluation datasets from the GLUE benchmark \cite{wang2018glue}, including WNLI, QNLI, QQP, and MRPC.
WNLI is a reading comprehension task.
% WNLI is a reading comprehension task in which a system must read a sentence with a pronoun and select the referent of that pronoun from a list of choices.
QNLI is a question-answering dataset consisting of question-paragraph pairs.
% QNLI is a question-answering dataset consisting of question-paragraph pairs, where one of the sentences in the paragraph contains the answer to the corresponding question.
QQP is a collection of question pairs from the community question-answering website Quora. 
MPRC is a corpus of sentence pairs automatically extracted from online news sources.
% MPRC is a corpus of sentence pairs automatically extracted from online news sources, with human annotations for whether the sentences in the pair are semantically equivalent.
For these four tasks, we report accuracy of the validation sets.
We also report the compression ratio on BERT by setting various \textit{N:M} configurations and quantized bitwidth of parameters.

% The second set and the third set are used to evaluate improvements on hardware optimizations.
% [Note] Chao Fang: 这个部分怎么提比较好呢？
% The second set evaluates hardware resource consumption of not only DMMEs, the core computing engine in the STA, at any common scale of \textit{N:M} sparsity, but also some representative STAs under various FPGA devices.
The second set dives into hardware resource consumption. 
Firstly, we study consumption of DMMEs, the core computing engine in the STA, at any common scale of \textit{N:M} sparsity, and then we explore hardware utilization of representative STAs under various FPGA devices.
For the former evaluation, DMMEs are not allowed to be synthesized using DSP blocks, which can be done by setting the property \textit{MAX\_DSP} as zero.
Hence, the consumption of LUTs and FFs can measure the cost of combinational logic and sequential logic for DMMEs, respectively.
The utilization of LUTs and FFs are reported at the synthesis stage as the metric of hardware resource requirements.
% The utilization of LUTs and FFs are reported at the synthesis stage as the metric of hardware resource requirements, where the consumption of LUTs and FFs can measure the cost of combinational logic and sequential logic for DMMEs, respectively.
% In this benchmark set, we synthesized a $4 \times 4$ unified MatMul computing engine as a simplified DMME with any common scale of \textit{N} and $M$ on Vivado 2021.2.
% For a fair comparison, these computing engines are not allowed to be synthesized using DSP blocks, which can be done by setting the property \textit{MAX\_DSP} as zero.
% We report the utilization of LUT and FF as the metric of hardware resource requirements, where LUT usage and FF usage can measure the consumption of combinational logic and sequential logic, respectively.
For the latter evaluation, the resource utilization of STAs on various FPGA devices are reported at the implementation stage, including the consuming amount of LUTs, FFs, BRAMs, and DSPs.

The third set studies performance improvements of overall STA hardware system on multiple FPGA platforms when deploying various Transformer-based models.
All key configurations of evaluated models in benchmark sets are presented in Table~\ref{tab:benchmark}.
At first, we evaluate the processing time with a single batch on all MHA and FFN ResBlocks in varying models from TinyBERT \cite{jiao2020tinybert}, Dino \cite{caron2021emerging}, and the Transformer-base model \cite{vaswani2017attention}.
% At first, we evaluate the processing time with a single batch on all MHA and FFN ResBlocks in varying Transformer-based models, which consist of TinyBERT \cite{jiao2020tinybert}, Dino \cite{caron2021emerging}, and the Transformer-base model \cite{vaswani2017attention}.
The selected models target different applications.
TinyBERT is a lightweight BERT model for many language tasks.
Dino, a tiny vision Transformer, can be the backbone for a lot of computer vision tasks.
Transformer-base model is the classic one for the neural machine translation (NMT) task.
Considering NMT is one of the sequence-to-sequence tasks, hence we split the Transformer-base model into two parts, the stacked encoders and decoders, respectively.
We finally make a fair comparison of the implemented STAs with previous works and commercial products using a shallow Transformer, which is the commonly used benchmark model in \cite{li2020ftrans,peng2021accelerating}.
Latency, throughput, power, energy efficiency and MAC efficiency are key metrics for applications, and thus used for performance evaluation.

% [Done] Chao Fang: 感觉这里应该插一个表格介绍模型的结构。
% [Note] 差评估的指标。以及 Shallow Transformer 的介绍

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[htbp]
\centering
\caption{Key configurations of Transformer-based models in benchmark sets}
\label{tab:benchmark}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
Benchmark                & Model                                                                       & \begin{tabular}[c]{@{}c@{}}Num. of \\ Encoders\end{tabular} & \begin{tabular}[c]{@{}c@{}}Num. of\\ Decoders\end{tabular} & \begin{tabular}[c]{@{}c@{}}Sequence \\ length\end{tabular} & \begin{tabular}[c]{@{}c@{}}Attention \\ heads\end{tabular} & \begin{tabular}[c]{@{}c@{}}Hidden\\ size\end{tabular} & \begin{tabular}[c]{@{}c@{}}Intermediate\\ size\end{tabular} \\ \midrule
Set I                    & BERT                                                                        & 12                                                          & 0                                                          & 128                                                              & 12                                                         & 768                                                   & 3072                                                        \\ \midrule
\multirow{10}{*}{Set III} & TinyBERT4                                                                   & 4                                                           & 0                                                          & 128                                                              & 12                                                         & 312                                                   & 1200                                                        \\ \cmidrule(l){2-8} 
                         & Dino-vits8                                                                  & 12                                                          & 0                                                          & 64                                                               & 6                                                          & 384                                                   & 1536                                                        \\ \cmidrule(l){2-8} 
                         & \begin{tabular}[c]{@{}c@{}}Transformer-base\\ stacked encoders\end{tabular} & 6                                                           & 0                                                          & 64                                                               & 8                                                          & 512                                                   & 2048                                                        \\ \cmidrule(l){2-8} 
                         & \begin{tabular}[c]{@{}c@{}}Transformer-base\\ stacked decoders\end{tabular} & 0                                                           & 6                                                          & 64                                                               & 8                                                          & 512                                                   & 2048                                                        \\ \cmidrule(l){2-8} 
                         & \begin{tabular}[c]{@{}c@{}}Shallow\\ Transformer\end{tabular}               & 2                                                           & 1                                                          & 64                                                               & 4                                                          & 200                                                   & 800                                                         \\ \bottomrule
\end{tabular}%
}
\end{table}

\subsubsection{\textbf{Implementation Details}} \label{subsec:impl}
~
\newline
\indent For algorithm implementation (Set I), the pre-trained models, the scripts and datasets are provided by the HuggingFace repository \cite{wolf2019huggingface}.
All models are implemented and executed using PyTorch v1.5.
% \cite{paszke2019pytorch}.

As for hardware implementation (Set II \& III), all modules of STA are designed in synthesizable SystemVerilog with the aid of hardware components from the BaseJump standard template library \cite{taylor2018basejump} and the PULP platform \cite{rossi2015pulp}.
Xilinx Vivado 2018.2 is the tool for synthesis and implementation.
We implement STA on three types of FPGA devices with various scales, including Xilinx ZYNQ Z7020 (XC7Z020), Xilinx Virtex-7 FPGA (XC7VX485T), and Xilinx UltraScale+ FPGA (XCVU13P).
Specifically, XC7Z020 is low-cost and low-resource System-on-Chip device equipped with a dual-core ARM Cortex-A9 processor and FPGA, which is fabricated in the 28 nm technology node.
XC7VX485T is a relatively large FPGA device fabricated in the 28 nm technology node.
XCVU13P, fabricated in the 16 nm technology node, is an extremely expensive and advanced FPGA device with abundant hardware resource.
% [Note] Chao Fang: 下面这一句还是挪到 baseline 比较好。因为这些实验是他们作为 baseline 的 platform，而不是我们实验所使用的 platform。
% For comparison with previous works and commercial products,
% [Note] Chao Fang: 这里是不是应该聊一聊为什么选用这三个平台的目的呢？

% \subsubsection{\textbf{Baseline}}
% ~
% \newline
% \indent 
% % For fair comparison, 

% % [Note] Chao Fang: 硬件的部分怎么说清楚比较好呢？在这一个 part 里，要讲清楚，Set II 是如何做的。Fig.14 是如何配置的？是如何选出来的这三个配置？Table II 又是如何配置的？
% % [Note] Chao Fang: 在 Set III 中，我们要提出来我们选取了哪些比较对象，这些比较对象的数据又是如何得到的。
% In benchmark set II, ...
% Following the comparison method in \cite{lu2021sanger}, we scale the size of computing engine in \cite{lu2020hardware}.
% To present scalability of STA, we 

% % [Note] Chao Fang: 这里的逻辑很乱，没有表达出想说的意思。
% As for benchmark set III, ARM Cortex-A57, Intel i9-9900X are CPU benchmarks.
% Jetson Nano and RTX 2080 Ti are GPU benchmarks.
% We also compare our STAs with prior FPGA-based works for accelerating Transformers, including \cite{lu2020hardware}, \cite{li2020ftrans}, and \cite{peng2021accelerating}.
% The dedicated accelerator in \cite{lu2020hardware}, equipped with a large 2D systolic array for dense operation, is the pioneer work for Transformer acceleration.
% FTRANS \cite{li2020ftrans}, is another recent specialized accelerator for Transformers, which exploits the speedup potential of block-circulant weight representations.
% In \cite{peng2021accelerating}, the proposed accelerator utilizes coarse-grained block-based sparsity to speedup Transformer inference.

% \textbf{Software implementation.} 
% We evaluate our methods on BERT \cite{kenton2019bert}, the well-known Transformer-based model. 
% Our four evaluation datasets come from the GLUE benchmark \cite{wang2018glue}, including WNLI, QNLI, QQP, and MRPC.
% For these four tasks, we report accuracy on the validation set, which is positively correlated with model accuracy.
% The pre-trained models, the scripts and datasets are provided by the HuggingFace repository \cite{wolf2019huggingface}.
% All models are implemented and executed using PyTorch v1.5 \cite{paszke2019pytorch}.
% Note that our pruning method use a pre-trained model as a start-point. 
% We directly finetune a pre-trained checkpoint on downstream tasks.
% For all tasks, we use a batch size of 32 and a initial learning rate of 2e-5.
% For WNLI, QNLI, QQP, there are 3 epochs to recover accuracy for every step of \textit{N}, while there are 5 epochs for MRPC.

% \textbf{Hardware implementation.}
% The STA is designed in synthesizable SystemVerilog with the aid of hardware components from the BaseJump standard template library \cite{taylor2018basejump} and the PULP platform \cite{rossi2015pulp}.

% \textbf{Platforms for comparison.}


\begin{figure*}[htb]
    \centering
    \subfloat[MNLI]{\includegraphics[width=0.21\linewidth]{figs/TVLSI-6-res-mnli.pdf}}
    \hfill
    \subfloat[QNLI]{\includegraphics[width=0.21\linewidth]{figs/TVLSI-6-res-qnli.pdf}}
    \hfill
    \subfloat[QQP]{\includegraphics[width=0.21\linewidth]{figs/TVLSI-6-res-qqp.pdf}}
    \hfill
    \subfloat[MRPC]{\includegraphics[width=0.21\linewidth]{figs/TVLSI-6-res-mrpc.pdf}}
    \caption{Pruning results on various tasks incluing (a) MNLI, (b) QNLI, (c) QQP, and (d) MRPC in comparison with ASP \cite{mishra2021accelerating} and SR-STE \cite{zhou2021learning}.}
    \label{fig:res_acc}
\end{figure*}

\subsection{Benchmark Set I: Algorithm Optimizations}
% \subsection{Eval. I: Comparing IDP to ASP and SRSTE}
% \subsection{Eval. II: Impact of Improved \textit{N} and Improved $M$}
% \subsection{Eval. III: Parameter Compression Ratio Considering Various Sparsity Configurations}

For benchmark set I, ASP \cite{mishra2021accelerating} and SR-STE \cite{zhou2021learning}, the two existing methods for acquiring \textit{N:M} sparse models, are selected as our baselines. 
The reported accuracy of baselines is obtained by training with released open-source code.
% [Note] Chao Fang: 这里如何讲清楚公平性呢？对于相同的 \textit{N:M} 配置，finetune 的 epoch 都是相同的。暂时用了下面的这个说法。
For a fair comparison, the generated \textit{N:M} sparse models using ASP, SR-STE, and our method are achieved with identical finetune epochs.
% Note that our pruning method use a pre-trained model as a start-point. 
% We directly finetune a pre-trained checkpoint on downstream tasks.
For all tasks, we use a batch size of 32 and a initial learning rate of 2e-5.
% [Note] Chao Fang: 下面这一句写的不够好，可能有歧义。等前文确定之后，我们再考虑后面怎么写清楚。
For WNLI, QNLI, QQP, there are 3 epochs to recover accuracy for every step of N, while there are 5 epochs for MRPC.

% [Note] Chao Fang: 这句话写的可能有点问题，后面需要继续修改、
% The pruning results on BERT \cite{kenton2019bert} are shown in Fig.~\ref{fig:res_acc}, applying to four representative tasks including MNLI, QNLI, QQP, and MRPC.
% We compare our method with two existing pruning method for \textit{N:M} sparsity pattern: NVIDIA ASP \cite{mishra2021accelerating} and SR-STE \cite{zhou2021learning}.
% For specific downstream tasks, we first finetune on the corresponding datasets to recover accuracy.
% [Note] Chao Fang: 这句话太废了，想想怎么改吧。
% And then, all three methods are evaluated using the same initial checkpoints and datasets.
% For fair comparison, points on the same x-axis are finetuned with the same epochs.

Compared with existing methods, Fig.~\ref{fig:res_acc} shows that IDP can achieve comparable or better accuracy under 75.00\% sparse ratio. In addition, the IDP can outperform the ASP and SR-STE method significantly with the sparse ratio increases. For instance, we can find that under 87.50\% (\textit{2:16}) sparse ratio, IDP consistently obtains large performance improvements to the baseline on all tasks ($5.36\%$ accuracy gain on MNLI, $10.38\%$ accuracy gain on QNLI, $2.98\%$ accuracy gain on QQP, and $8.08\%$ accuracy gain on MRPC). Therefore, we can obtain the state-of-the-art \textit{N:M} sparse models for FPGA-based platform deployment with the plug-and-play IDP algorithm. 

% Fig.~\ref{fig:res_comp} presents the trade-off between model sparsity and model compression ratio.

Based on our evaluations of model accuracy with respect to parameter
sparsity, as shown in Fig.~\ref{fig:res_acc}, it is observed that Transformers can hardly achieve a sparsity over $90\%$ without impacting accuracy. It would be more likely practical for \textit{N:M} sparse Transformers with a sparsity ranging from $50\%$ to $87.5\%$.
Next, BERT is taken as an example to evaluate the storage reduction of our compression scheme when using multiple quantized bits under various \textit{N:M} sparsity configurations.
We make a elaborated comparison between our bitmap-based scheme, COO, CSR, CSC, and step indexing \cite{zhang2016cambricon}.
Compared with the other mainstream methods, as shown in Fig.~\ref{fig:res_comp}, our scheme can achieve the highest compression ratio when the model sparsity is varied from $50\%$ to $87.5\%$.
The compression ratio keeps increasing as the model sparsity increases. 
An \textit{N:M} sparse BERT, can achieve a higher compression ratio when quantized in larger bit widths.
BERT with 50.00\% \textit{N:M} sparsity can reach a $1.78\times$ reduction on storage of parameters.
When BERT has a sparsity of 87.50\%, it achieves a significant storage saving, up to $5.33\times$, on parameters.
Our compression scheme can efficiently reduce the storage requirement for \textit{N:M} sparse parameters.
In subsequent hardware evaluations, we uniformly adopt a 16-bit fixed-point representation for Transformers to avoid negative impacts on model accuracy due to quantization.

\begin{figure}[htb]
    \centering
    \subfloat[Bitwidth = 4bit]{\includegraphics[width=0.23\textwidth]{figs/r1_TVLSI-6-res-compression-bw4.pdf}}
    \subfloat[Bitwidth = 8bit]{\includegraphics[width=0.23\textwidth]{figs/r1_TVLSI-6-res-compression-bw8.pdf}}
    \\
    \subfloat[Bitwidth = 16bit]{\includegraphics[width=0.23\textwidth]{figs/r1_TVLSI-6-res-compression-bw16.pdf}}
    \subfloat[Bitwidth = 32bit]{\includegraphics[width=0.23\textwidth]{figs/r1_TVLSI-6-res-compression-bw32.pdf}}
    \caption{\RoundOne{Compression ratio on BERT with various sparsity configurations.}}
    \label{fig:res_comp}
\end{figure}

% \begin{figure} [htbp] 
% 	\centering
% 	\includegraphics[width=0.48\textwidth]{figs/TVLSI-6-res-compression.pdf}
% 	\caption{Compression ratio on BERT with various sparsity configurations.} 
% 	\label{fig:res_comp}
% \end{figure}

\subsection{Benchmark Set II: Hardware Resource Consumption}

% The second benchmark set is used to examine the hardware resource consumption of STA.

The second benchmark set verifies hardware consumption of STAs that have not yet deployed Transformer models.

At first, we evaluate the hardware requirements of DMME in common sparse configurations by comparing it against multiple dense computing engines.
% Then, we evaluate hardware resource consumption of STA on three types of FPGAs platforms.
% For a fair comparison, all evaluated computing engines are synthesized as a $4 \times 4$ unified MatMul computing engine, while PEs are configured in various common scale of \textit{N} and $M$.
For a fair comparison, evaluated computing engines are all synthesized as a $2 \times 2$ unified MatMul computing engine
% , that is, $H=1, R=C=2$
, and only PEs in these engines are configured into various \textit{N:M} configurations.
% For a fair comparison, evaluated computing engines are all synthesized on Vivado 2018.2 as a $4 \times 4$ unified MatMul computing engine, that is, $H=1, R=C=4$, and only PEs in these engines are configured into various \textit{N:M} configurations.
Note that those computing engines that make \textit{N} equal to \textit{M}, exclude the non-zero element selectors and merely support dense computing.
It can be regarded as the computing engine in \cite{lu2020hardware} if both \textit{N} and \textit{M} are \textit{1} in the evaluated DMME.
% In our experiment, \textit{N} is ranged from 1 to 3, and $M$ is selected from 2, 4, 8, and 16.
% For simplicity, we synthesized a $4 \times 4$ unified MatMul computing engine as DMME with any common scale of \textit{N} and $M$ on Vivado 2021.2.
These computing engines are not allowed to be synthesized using DSP blocks, which can be done by setting the property \textit{MAX\_DSP} as zero.
Hence, the utilization of LUTs and FFs from Vivado synthesis reports can be used to measure the consumption of combinational logic and sequential logic for DMMEs, respectively.

Fig.~\ref{fig:res_area} presents the comparison of required hardware resource consumption between DMMEs of various configurations.
For simplicity, all results are normalized to the \textit{4:4} dense baseline computing engine.
Gray bars 
% in Fig.~\ref{fig:res_area} 
are resource consumption of various computing engines with sole support on dense matrix multiplication.
Green, red, and yellow bars represent hardware utilization of DMMEs, when \textit{N} is set as 1, 2, and 3, respectively.
% For instance, PEs in \textit{2:2} baseline computing engine merely support dense dot product with a length of 2 in a cycle.
% Nevertheless, PEs in the \textit{2:8} DMME can not only perform a \textit{2}-length dense dot product, but also a \textit{8}-length sparse dot product that has 2 valid terms.
In Fig.~\ref{fig:res_area}, we can observe hardware resource saved by DMMEs compared to dense baseline computing engine under sparse matrix computing mode.
When $M=16$ and \textit{N} is set to 1, 2, and 3, respectively, DMME, in contrast to \textit{16:16} baseline, obtains saving of combinational logic up to $7.96 \times$, $4.76 \times$, and $3.17 \times$ , while achieving reduction on sequential logic $4.41\times$, $2.63\times$, and $1.99\times$.
% According to Fig.~\ref{fig:res_area}, when $M=16$ and \textit{N} is set to 1, 2, and 3, respectively, DMME, in contrast to $16:16$ baseline, obtains saving of combinational logic up to $7.96 \times$, $4.76 \times$, and $3.17 \times$ , while achieving reduction on sequential logic $4.41\times$, $2.63\times$, and $1.99\times$.
% Note that \textit{3:4} DMME, compared with \textit{4:4} baseline, has merely an $8\%$ reduction on combinational logic with an $11\%$ additional cost of sequential logic.
% It reveals that if targeted sparsity is too low, DMME will consume more hardware resources, which is inefficient, to support sparse computing.
% If the sparsity is greater than $50\%$, DMMEs can achieve significant savings of hardware resource consumption in contrast to baseline computing engines under the same effective throughput for sparse computing.
% We then study the increased hardware resource consumption of DMME compared to baseline computing engines under dense matrix computing mode.
% As shown in Fig.~\ref{fig:res_area}, when $N=3$ and $M$ is set to 4, 8, and 16, respectively, DMME has $18\%$, $32\%$, and $58\%$ extra cost on combinational logic, and $48\%$, $64\%$, and $136\%$ overhead of sequential logic.
% The hardware savings in the sparse matrix computation mode is more of concern than the increase in the dense matrix computation mode, since sparse-dense matrix multiplication with parameters dominates operations, approximately up to 90\%, in both the MHA module and the FFN module.
According to Fig.~\ref{fig:res_area}, we further evaluate the impact of separately increasing \textit{N} and \textit{M} in DMMEs on hardware resource consumption.
For instance, \textit{3:4} DMME costs $2.42\times$ combinational logic and $2.78\times$ sequential logic of \textit{1:4} DMME.
However, \textit{1:16} DMME merely requires $1.28\times$ combinational logic and $2.00\times$ sequential logic over \textit{1:4} DMME.
% Hence, increasing \textit{M} requires less hardware resource overhead than increasing \textit{N} for DMMEs.

\begin{figure}[htb]
    \centering
    \subfloat[Combinational logic]{
        \includegraphics[width=0.23\textwidth]{figs/r1_TVLSI-6-res-2x2_array_area_report_LUT.pdf}
    }
    % \\
    \subfloat[Sequential logic]{
        \includegraphics[width=0.23\textwidth]{figs/r1_TVLSI-6-res-2x2_array_area_report_FF.pdf}
    }
    \caption{The normalized resource consumption of unified computing engine over the classic computing engine on various scales including (a) combinational logic and (b) sequential logic.}
    \label{fig:res_area}
\end{figure}

% [Note] Chao Fang: 关于图 14 的四点：
% 1. 稠密矩阵计算引擎改进成稀疏矩阵计算引擎的 overhead
% 2. 稀疏矩阵计算引擎改进后与稠密矩阵计算相比的 performance improvement
% 3. 增加 \textit{M} 带来的面积增益
% 4. 增加 \textit{N} 带来的面积增益
% We first report the resource consumption of DMME with multiple common scales, including combinational logic and sequential logic.
% As shown in Fig.~\ref{fig:res_area}, 

We finally evaluate hardware resource consumption of STA on three types of FPGA platforms, including XC7Z020, XC7VX485T, and XCVU13P.
These FPGA platforms are used to represent diverse devices in Fig.~\ref{fig:model_overview}.
Considering the hardware resource and cost on these platforms, we intend to deploy XC7Z020 to the edge and XC7VX485T and XCVU13P on the clouds.
There are many tunable parameters of STAs, especially in DMME, which have great impacts on performance.
In order to determine the specific parameters of STA on each FPGA platforms, we design a cycle-accurate simulator to evaluate actual inference performance based on the given specifications.
STA in XC7Z020 adopts an aggressive \textit{1:8} sparsity since latency is the critical metric on the edge platforms.
However, STAs in both XC7VX485T and XCVU13P configured \textit{N:M} as \textit{2:8} because devices deployed on the clouds concerns latency as well as model accuracy.
Table~\ref{tab:util} shows resource consumption of STAs deployed on three scales of FPGA platforms, namely STA-Tiny, STA-Small, and STA-Large, respectively.
\RoundOne{
The FPGA resource and power breakdown of STA-Small are presented in Table~\ref{tab:breakdown}.
The \textit{N}-parallel MAC (N-MAC) module dominates the DSP consumption of STA since it is the core of computing engine for MAC operations.
The non-zero element selector (NZES) module takes the majority of LUT consumption due to the cost for decoding and index selection.
The routing module occupies most registers of DMME for datapath selection and temporary data storage.
Moreover, the proposed DMME and softmax module occupy $47.29\%$ and $9.42\%$ power consumption, respectively.
}
% [TBD] Chao Fang: Needs data to complement...

% \subsection{Eval. IV: Area Overhead of DMME and Improved Computational Efficiency}

% We start by measuring the area-throughput trade-offs of STA by scaling its \textit{N} and $M$.
% For simplicity, we synthesized a $4 \times 4$ unified MatMul computing engine with any common scale of \textit{N} and $M$ on Vivado 2021.2.
% For a fair comparison, these computing engines are not allowed to be synthesized using DSP blocks, which can be done by setting the property \textit{MAX\_DSP} as zero.
% Therefore, we report the utilization of LUT and FF as the area metric.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[htb]
\centering
\caption{FPGA resource utilization}
\label{tab:util}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}c|ccccc@{}}
\toprule
Platform                                                            & Frequency & LUT                                                   & FF                                                    & BRAM                                                  & DSP                                                   \\ \midrule
\begin{tabular}[c]{@{}c@{}}1:8 STA-Tiny\\ (XC7Z020)\end{tabular}    & 150MHz  
% & 21,486 & 75,763 & 96 & 132 \\ \midrule
% & \begin{tabular}[c]{@{}c@{}} 21,486\\ (40.38\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 75,763\\ (71.21\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 96\\ (68.57\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 132\\ (60.00\%)\end{tabular} \\ \midrule
& \begin{tabular}[c]{@{}c@{}} 21K \\ (40.38\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 75K \\ (71.21\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 96\\ (68.57\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 132\\ (60.00\%)\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}c@{}}2:8 STA-Small\\ (XC7VX485T)\end{tabular} & 200MHz
% & 116,640 & 337,116 & 532 & 1,040 \\ \midrule
% & \begin{tabular}[c]{@{}c@{}} 116,640\\ (38.42\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 337,116\\ (55.52\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 532\\ (51.65\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 1,040\\ (37.14\%)\end{tabular} \\ \midrule
& \begin{tabular}[c]{@{}c@{}} 116K\\ (38.42\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 337K\\ (55.52\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 532\\ (51.65\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 1,040\\ (37.14\%)\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}c@{}}2:8 STA-Large\\ (XCVU13P)\end{tabular}   & 200MHz
% & 464,545 & 1,321,437  & 1,192 & 4,160 \\ \bottomrule
% & \begin{tabular}[c]{@{}c@{}} 464,545\\ (26.88\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 1,321,437\\ (38.24\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 1,192\\ (44.35\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 4,160\\ (33.85\%)\end{tabular} \\ \bottomrule
& \begin{tabular}[c]{@{}c@{}} 464K\\ (26.88\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 1,321K\\ (38.24\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 1,192\\ (44.35\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}} 4,160\\ (33.85\%)\end{tabular} \\ \bottomrule
\end{tabular}%
}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% FE0000 / 000000
% \begin{table}[bht]
% \centering
% \caption{\RoundOne{FPGA Resource and Power Breakdown of STA-Small}}
% \label{tab:breakdown}
% \resizebox{0.46\textwidth}{!}{%
% \begin{tabular}{@{}cc|ccccc@{}}
% \toprule
% \multicolumn{2}{c|}{{\color[HTML]{000000} }}                                                        & {\color[HTML]{FE0000} LUT}                                                              & {\color[HTML]{FE0000} FF}                                                                & {\color[HTML]{FE0000} BRAM}                                                             & {\color[HTML]{FE0000} DSP}                                                               & {\color[HTML]{FE0000} Power (W)}                                                         \\ \midrule
% \multicolumn{1}{c|}{{\color[HTML]{FE0000} }}                       & {\color[HTML]{FE0000} N-MAC}   & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}16K\\ (13.79\%)\end{tabular}}          & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}66K\\ (19.58\%)\end{tabular}}           & {\color[HTML]{FE0000} \textbf{-}}                                                       & {\color[HTML]{FE0000} \textbf{\begin{tabular}[c]{@{}c@{}}1024\\ (98.46\%)\end{tabular}}} & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}2.78\\ (28.17\%)\end{tabular}}          \\ \cmidrule(l){2-7} 
% \multicolumn{1}{c|}{{\color[HTML]{FE0000} }}                       & {\color[HTML]{FE0000} NZES}    & {\color[HTML]{FE0000} \textbf{\begin{tabular}[c]{@{}c@{}}66K\\ (56.90\%)\end{tabular}}} & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}70K\\ (20.77\%)\end{tabular}}           & {\color[HTML]{FE0000} -}                                                                & {\color[HTML]{FE0000} -}                                                                 & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}0.83\\ (8.41\%)\end{tabular}}           \\ \cmidrule(l){2-7} 
% \multicolumn{1}{c|}{\multirow{-6}{*}{{\color[HTML]{FE0000} DMME}}} & {\color[HTML]{FE0000} Routing} & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}9K\\ (7.76\%)\end{tabular}}            & {\color[HTML]{FE0000} \textbf{\begin{tabular}[c]{@{}c@{}}180K\\ (53.41\%)\end{tabular}}} & {\color[HTML]{FE0000} -}                                                                & {\color[HTML]{FE0000} -}                                                                 & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}1.06\\ (10.74\%)\end{tabular}}          \\ \midrule
% \multicolumn{2}{c|}{{\color[HTML]{FE0000} Softmax}}                                                 & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}13K\\ (11.21\%)\end{tabular}}          & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}8K\\ (2.37\%)\end{tabular}}             & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}16\\ (3.00\%)\end{tabular}}            & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}16\\ (1.54\%)\end{tabular}}             & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}0.93\\ (9.42\%)\end{tabular}}           \\ \midrule
% \multicolumn{2}{c|}{{\color[HTML]{FE0000} Others}}                                                  & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}12K\\ (10.34\%)\end{tabular}}          & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}13K\\ (3.86\%)\end{tabular}}            & {\color[HTML]{FE0000} \textbf{\begin{tabular}[c]{@{}c@{}}516\\ (97.00\%)\end{tabular}}} & {\color[HTML]{FE0000} \textbf{-}}                                                        & {\color[HTML]{FE0000} \textbf{\begin{tabular}[c]{@{}c@{}}4.27\\ (43.26\%)\end{tabular}}} \\ \midrule
% \multicolumn{2}{c|}{{\color[HTML]{FE0000} Total}}                                                   & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}116K\\ (100.00\%)\end{tabular}}        & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}337K\\ (100.00\%)\end{tabular}}         & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}532\\ (100.00\%)\end{tabular}}         & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}1040\\ (100.00\%)\end{tabular}}         & {\color[HTML]{FE0000} \begin{tabular}[c]{@{}c@{}}9.87\\ (100.00\%)\end{tabular}}         \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[bht]
\centering
\caption{\RoundOne{FPGA Resource and Power Breakdown of STA-Small}}
\label{tab:breakdown}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}cc|ccccc@{}}
\toprule
\multicolumn{2}{c|}{{\color[HTML]{000000} }}                                                        & {\color[HTML]{000000} LUT}                                                              & {\color[HTML]{000000} FF}                                                                & {\color[HTML]{000000} BRAM}                                                             & {\color[HTML]{000000} DSP}                                                               & {\color[HTML]{000000} Power (W)}                                                         \\ \midrule
\multicolumn{1}{c|}{{\color[HTML]{000000} }}                       & {\color[HTML]{000000} N-MAC}   & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}16K\\ (13.79\%)\end{tabular}}          & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}68K\\ (20.18\%)\end{tabular}}           & {\color[HTML]{000000} \textbf{-}}                                                       & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}1024\\ (98.46\%)\end{tabular}}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}2.78\\ (28.17\%)\end{tabular}}          \\ \cmidrule(l){2-7} 
\multicolumn{1}{c|}{{\color[HTML]{000000} }}                       & {\color[HTML]{000000} NZES}    & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}66K\\ (56.90\%)\end{tabular}}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}68K\\ (20.18\%)\end{tabular}}           & {\color[HTML]{000000} -}                                                                & {\color[HTML]{000000} -}                                                                 & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}0.83\\ (8.41\%)\end{tabular}}           \\ \cmidrule(l){2-7} 
\multicolumn{1}{c|}{\multirow{-6}{*}{{\color[HTML]{000000} DMME}}} & {\color[HTML]{000000} Routing} & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}9K\\ (7.76\%)\end{tabular}}            & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}180K\\ (53.41\%)\end{tabular}}} & {\color[HTML]{000000} -}                                                                & {\color[HTML]{000000} -}                                                                 & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}1.06\\ (10.74\%)\end{tabular}}          \\ \midrule
\multicolumn{2}{c|}{{\color[HTML]{000000} Softmax}}                                                 & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}13K\\ (11.21\%)\end{tabular}}          & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}8K\\ (2.37\%)\end{tabular}}             & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}16\\ (3.00\%)\end{tabular}}            & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}16\\ (1.54\%)\end{tabular}}             & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}0.93\\ (9.42\%)\end{tabular}}           \\ \midrule
\multicolumn{2}{c|}{{\color[HTML]{000000} Others}}                                                  & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}12K\\ (10.34\%)\end{tabular}}          & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}13K\\ (3.86\%)\end{tabular}}            & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}516\\ (97.00\%)\end{tabular}}} & {\color[HTML]{000000} \textbf{-}}                                                        & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}4.27\\ (43.26\%)\end{tabular}}} 
\\ \midrule
\multicolumn{2}{c|}{{\color[HTML]{000000} Total}}                                                   & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}116K\\ (100.00\%)\end{tabular}}        & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}337K\\ (100.00\%)\end{tabular}}         & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}532\\ (100.00\%)\end{tabular}}         & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}1040\\ (100.00\%)\end{tabular}}         & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}9.87\\ (100.00\%)\end{tabular}}         
\\ \bottomrule
\end{tabular}%
}
\end{table}

\subsection{Benchmark Set III: Overall System Evaluation}

The third benchmark set is used to evaluate performance when deploying various Transformer-based models on STAs.

Firstly, we study the inference speedup of STAs by contrast with CPUs, GPUs, and the prior dedicated accelerators.
The selected models to be deployed are composed of TinyBERT \cite{jiao2020tinybert}, Dino \cite{caron2021emerging}, the classic Transformer model \cite{vaswani2017attention}.
Here we consider single-batch processing time in all the MHA and FFN ResBlocks of these Transformer-based models. 
For cross-platform comparison, the hardware setup is as follows to execute the Transformer inference tasks.
The CPU results are measured using an ARM Cortex A57 and an Intel i9-9900X.
The former commonly appeared in mobile devices for edge applications, while the latter is a high-end CPU product for deploying cloud applications.
\RoundOne{The GPU results are measured using an NVIDIA Jeston Nano, an embedded GPU product for edge applications, an NVIDIA RTX 2080Ti, and an NVIDIA RTX 3090 capable of 2:4 sparse acceleration.}
% All CPU and GPU results are evaluated under the PyTorch framework.
Following the comparison method in \cite{lu2021sanger}, we apply \cite{lu2020hardware} as baselines on FPGA platforms by scaling the size of its computing engine.
\RoundOne{Two existing sparse accelerators for Transformers, OPTIMUS \cite{park2020optimus} and EdgeBERT \cite{tambe2021edgebert}, are evaluated as well for a more comprehensive comparison of STA.}
% In other words, baselines, namely Tiny, Small and Large, have the same number of MACs in the core computing engine as their STA counterparts.
% In addition, their operating frequency is also consistent with the corresponding STAs.
% Moreover, we additionally employ models on all STAs in non-sparse mode, to observe the improvement on hardware optimization.
Fig.~\ref{fig:res_latency} shows the idealized performance speedup of different hardware platforms, where edge and cloud platforms normalized to the ARM Cortex A57 and Intel i9-9900X, respectively.

\begin{figure}[bht]
    \centering
    \subfloat[]{
        \includegraphics[width=0.48\textwidth]{figs/r1_TVLSI-6-res-time_comsumption_edge.pdf}
        \label{fig:res_edge_latency}
    }
    \\
    \subfloat[]{
        \includegraphics[width=0.48\textwidth]{figs/r1_TVLSI-6-res-time_comsumption_cloud.pdf}
        \label{fig:res_cloud_latency}
    }
    \caption{\RoundOne{The processing time of Transformer-based models on various (a) edge platforms and (b) cloud platforms.}}
    \label{fig:res_latency}
\end{figure}

As shown in Fig.~\ref{fig:res_latency}~(a), among all edge platforms, STA-Tiny achieves a geometric mean increase of $32.96\times$, $2.69\times$, and $5.38 \times$ over CPU, GPU, and the FPGA baseline, respectively.
% When only activated in dense mode, STA-Tiny still has better performance improvement than the FPGA baseline.
% This is due to an elaborate exploit in DMME for head parallelism in Transformer-based models by contrast with the FPGA baseline \cite{lu2020hardware}, which effectively reduces inference latency of DMME.
% Furthermore, STA-Tiny can achieve $5.13\times$ additional speedup if enabling both dense mode and sparse mode for computing.
Fig.~\ref{fig:res_latency}~(b) presents the performance comparison between various cloud platforms.
% Compared to CPU and GPU platforms, STA-Small achieves $4.32\times$ and $1.38\times$ performance improvements, respectively, while STA-Large reaches significant speedup up to $13.19\times$ and $4.21\times$, respectively.
% Note that STA-Small achieves comparable inference latency to the large baseline, where STA-Small utilizes merely a quarter number of MACs of the large baseline.
% STA-Small and STA-Large significantly exceed the baseline counterparts even only used under dense mode for computing.
% When both dense mode and sparse mode are activated, STA-Small and STA-Large achieve $2.90\times$ and $2.65\times$ performance improvements, respectively, in contrast with the corresponding FPGA baselines.
\RoundOne{
For fair comparison, Baseline-Small (red), EdgeBERT (purple), OPTIMUS (brown), and \textit{2:8} STA-Small (pink) in Fig.~\ref{fig:res_latency}~(b) are evaluated under the same number of MAC units and clock frequency.
% Let's focus on the Baseline-Small (red), EdgeBERT (purple), OPTIMUS (brown), and 2:8 STA-Small (pink) in Fig.~\ref{fig:resp_rev2_cloud}.
% All of them are evaluated under the same number of MAC units and clock frequency.
% Moreover, the weight parameters are all pruned with a sparsity up to $75\%$.
% The baseline performs operations of Transformer by a large 2D systolic array
}
\RoundOne{
% [Chao Fang] 这个部分可能表述的有点问题，尤其是在创新的划分上。
\begin{itemize}
    \item \textbf{STA v.s. Baseline-Small} \cite{lu2020hardware}: 
    \textit{2:8} STA-Small achieves $2.89\times$ speedup on average over Baseline-Small, which enables dense Transformer acceleration using a large 2D systolic array.
    % Baseline-Small is not in favor of sparse operations, merely performs dense Transformer using a large 2D systolic array.
    It suffers low utilization of MAC units due to inflexible mapping scheme and large skew latency for systolic-arranged data. 
    STA achieves significant performance improvement by: 1) innovation of DMME from the architectural aspects, and 2) reduction on MAC operations of \textit{N:M} sparse Transformers from the algorithmic aspects.
    We further present a performance breakdown of STA compared to Baseline-Small.
    As shown in Fig.~\ref{fig:sta_small_perf}, the architectural innovation for DMME can achieve $1.08\times$ better performance improvement, and there is $2.68\times$ speedup on top of the architectural innovation by efficiently enabling \textit{2:8} sparse acceleration.
    \item \textbf{STA v.s. EdgeBERT} \cite{tambe2021edgebert}:
    \textit{2:8} STA-Small achieves $2.33\times$ speedup on average over EdgeBERT-32, which is an energy-optimized Transformer accelerator exploiting unstructured sparsity.
    % . EdgeBERT is an energy-optimized Transformer accelerator, which exploits unstructured sparsity in both input and weight matrices.
    % Its processing unit takes two $n \times n$ matrices as input and computes $n^3$ MAC operations in $n$ clock cycles.
    When performing sparse MAC operations, processing units of EdgeBERT skip the zero input value through a gating strategy, which can significantly reduce energy consumption, but offer little benefit to latency.
    Compared to EdgeBERT, STA performs \textit{N:M} sparse MAC operations by choosing non-zero inputs, which can both reduce energy and optimize latency.
    \item \textbf{STA v.s. OPTIMUS} \cite{park2020optimus}:
    \textit{2:8} STA-Small has a $1.20\times$ better performance on average over OPTIMUS, which is a high performance sparse accelerator for Transformers exploiting unstructured sparsity in weight parameters. 
    % . OPTIMUS is a high performance sparse accelerator for Transformers, which exploit unstructured sparsity in weight parameters.
    % Its computing engine, composed of 1024 MAC units, is orchestrated in 1D vector array. 
    When performing sparse MAC operations, OPTIMUS can hardly achieve high MAC utilization due to load imbalance and input load miss.
    % [Chao Fang] 感觉这里还是要详细解释一下。
    STA can effectively overcome these two problem suffered by OPTIMUS.
    STA gets rid of load imbalance by arranging each MAC in DMME to perform operations in a balanced \textit{N:M} group.
    In addition, STA loads a series of input \textit{N:M} groups at each cycle, and utilizes these elements multiple times in a systolic manner, which effectively addresses input load miss compared to OPTIMUS.
    % The \textit{N:M} group-based sparsity can guarantee every 
\end{itemize}
}

% \begin{figure*}[bht]
%     \centering
%     \subfloat[]{
%         \includegraphics[width=0.45\textwidth]{figs/r1_TVLSI-6-res-time_comsumption_edge.pdf}
%         \label{fig:res_edge_latency}
%     }
%     \subfloat[]{
%         \includegraphics[width=0.50\textwidth]{figs/r1_TVLSI-6-res-time_comsumption_cloud.pdf}
%         \label{fig:res_cloud_latency}
%     }
%     \caption{The processing time of Transformer-based models on various (a) edge platforms and (b) cloud platforms.}
%     \label{fig:res_latency}
% \end{figure*}

\begin{figure} [tbp] 
	\centering
	\includegraphics[width=0.46\textwidth]{figs/r1_TVLSI-6-res-op_rt_breakdown.pdf}
	\caption{\RoundOne{Performance and MAC operation breakdown of STA-Small.}}
	\label{fig:sta_small_perf}
\end{figure}

% In this section, we first evaluate the speedup of STAs over other benchmarks with Transformer-based models considered in Fig.~\ref{fig:res_latency}.
% ARM Cortex-A57, Intel i9-9900X are CPU benchmarks.
% Jetson Nano and RTX 2080 Ti are GPU benchmarks.

% \begin{table*}[t]
% \centering
% \caption{Comparison of STAs with previous works and commercial products}
% \label{tab:perf_cmp}
% \resizebox{0.92\textwidth}{!}{%
% \begin{tabular}{@{}c|ccccccccc@{}}
% \toprule
% \multirow{4}{*}{Platform}   & \multicolumn{1}{c|}{CPU}                       & \multicolumn{2}{c|}{GPU}                                                         & \multicolumn{6}{c}{FPGA}                                                                                                                  \\ \cmidrule(l){2-10} 
%                             & \multicolumn{1}{c|}{\multirow{2}{*}{i9-9900X}} & \multirow{2}{*}{Jetson Nano} & \multicolumn{1}{c|}{\multirow{2}{*}{RTX 2080 Ti}} & \multirow{2}{*}{SOCC'20 \cite{lu2020hardware}} & \multirow{2}{*}{ISLPED'20 \cite{li2020ftrans}} & \multicolumn{1}{c|}{\multirow{2}{*}{ISQED'21 \cite{peng2021accelerating}}} & \multicolumn{3}{c}{Our work}     \\ \cmidrule(l){8-10} 
%                             & \multicolumn{1}{c|}{}                          &                              & \multicolumn{1}{c|}{}                             &                          &                            & \multicolumn{1}{c|}{}                          & STA-Tiny & STA-Small & STA-Large \\ \midrule
% Chip                        & \multicolumn{1}{c|}{Skylake}                   & Tegra X1                     & \multicolumn{1}{c|}{TU102}                        & XCVU13P                  & XCVU9P                     & \multicolumn{1}{c|}{XCU200}                    & XC7Z020  & XC7VX485T & XCVU13P   \\ \midrule
% Technology                  & \multicolumn{1}{c|}{14 nm}                     & 20 nm                        & \multicolumn{1}{c|}{12 nm}                        & 16 nm                    & 16 nm                      & \multicolumn{1}{c|}{16 nm}                     & 28 nm    & 28 nm     & 16 nm     \\ \midrule
% Frequency                   & \multicolumn{1}{c|}{3.50 GHz}                  & 640 MHz                      & \multicolumn{1}{c|}{1.35 GHz}                     & 200 MHz                  & -                          & \multicolumn{1}{c|}{-}                         & 150 MHz  & 200 MHz   & 200 MHz   \\ \midrule
% \# MAC units                & \multicolumn{1}{c|}{-}                         & -                            & \multicolumn{1}{c|}{-}                            & 4096                     & $\sim$ 5647                & \multicolumn{1}{c|}{$\sim$ 3368}               & 128      & 1024      & 4096      \\ \midrule
% Bit Precision               & \multicolumn{1}{c|}{FP-32}                     & FP-32                        & \multicolumn{1}{c|}{FP-32}                        & FIX-8                    & FIX-16                     & \multicolumn{1}{c|}{-}                         & \multicolumn{3}{c}{FIX-16}       \\ \midrule
% Test Network                & \multicolumn{9}{c}{Shallow Transformer}                                                                                                                                                                                                                                       \\ \midrule
% Latency (ms)                & \multicolumn{1}{c|}{2.17}                      & 16.24                        & \multicolumn{1}{c|}{1.70}                         & 0.30                     & 2.94                       & \multicolumn{1}{c|}{0.32}                      & 2.01     & 0.42      & 0.15      \\ \midrule
% Batch-1 Throughput (GOP/s)  & \multicolumn{1}{c|}{101.38}                    & 13.55                        & \multicolumn{1}{c|}{129.41}                       & 733.33                   & 75.34                      & \multicolumn{1}{c|}{687.50}                    & 109.45   & 523.81    & 1466.67   \\ \midrule
% Power (W)                   & \multicolumn{1}{c|}{165.00}                    & 7.56                         & \multicolumn{1}{c|}{250.00}                       & 16.70                    & 22.45                      & \multicolumn{1}{c|}{-}                         & 2.71      & 9.87       & 26.59       \\ \midrule
% Energy Efficiency (GOP/J)   & \multicolumn{1}{c|}{0.61}                      & 1.79                         & \multicolumn{1}{c|}{0.52}                         & 43.91                    & 3.35                       &   \multicolumn{1}{c|}{-}                         & 40.39     & 53.07      & 55.16       \\ \midrule
% MAC Efficiency (GOP/s/unit) & \multicolumn{1}{c|}{-}                         & -                            & \multicolumn{1}{c|}{-}                            & 0.18                     & $\sim$ 0.01                & \multicolumn{1}{c|}{$\sim$ 0.20}               & 0.86     & 0.51      & 0.36      \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}  

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table*}[t]
% \centering
% \caption{Comparison of STAs with previous works and commercial products.}
% \label{tab:perf_cmp}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}c|ccccccccc@{}}
% \toprule
% \multirow{4}{*}{Platform}   & CPU                                            & \multicolumn{2}{|c|}{GPU}                                                          & \multicolumn{6}{c}{FPGA}                                                                                                                                                                                                                                                                                                                                      \\ \cmidrule(l){2-10} 
%                             & \multicolumn{1}{c|}{\multirow{2}{*}{i9-9900X}} & \multirow{2}{*}{Jetson Nano} & \multicolumn{1}{c|}{\multirow{2}{*}{RTX 2080 Ti}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}SOCC'20\\ \cite{lu2020hardware}\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ISLPED'20\\ \cite{li2020ftrans}\end{tabular}} & \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ISQED'21\\ \cite{peng2021accelerating}\end{tabular}}} & \multicolumn{3}{c}{Our work}                \\ \cmidrule(l){8-10} 
%                             & \multicolumn{1}{c|}{}                          &                              & \multicolumn{1}{c|}{}                             &                                                                                             &                                                                                               & \multicolumn{1}{c|}{}                                                                                             & STA-Tiny     & STA-Small     & STA-Large    \\ \midrule
% Chip                        & \multicolumn{1}{c|}{Skylake}                   & Tegra X1                     & \multicolumn{1}{c|}{TU102}                        & XCVU13P                                                                                     & XCVU9P                                                                                        & \multicolumn{1}{c|}{XCU200}                                                                                       & XC7Z020      & XC7VX485T     & XCVU13P      \\ \midrule
% Technology                  & \multicolumn{1}{c|}{14 nm}                     & 20 nm                        & \multicolumn{1}{c|}{12 nm}                        & 16 nm                                                                                       & 16 nm                                                                                         & \multicolumn{1}{c|}{16 nm}                                                                                        & 28 nm        & 28 nm         & 16 nm        \\ \midrule
% Frequency                   & \multicolumn{1}{c|}{3.50 GHz}                  & 640 MHz                      & \multicolumn{1}{c|}{1.35 GHz}                     & 200 MHz                                                                                     & -                                                                                             & \multicolumn{1}{c|}{-}                                                                                            & 150 MHz      & 200 MHz       & 200 MHz      \\ \midrule
% Methods                     & \multicolumn{1}{c|}{-}                         & -                            & \multicolumn{1}{c|}{-}                            & \begin{tabular}[c]{@{}c@{}}Low-bit\\ quantization\end{tabular}                              & \begin{tabular}[c]{@{}c@{}}Block-circulant\\ matrix with FFT\end{tabular}                     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Block-based\\ pruning\end{tabular}}                                & \multicolumn{3}{c}{\textit{N:M} group-based pruning} \\ \midrule
% \# MAC units                & \multicolumn{1}{c|}{-}                         & -                            & \multicolumn{1}{c|}{-}                            & 4096                                                                                        & $\sim$ 5647                                                                                   & \multicolumn{1}{c|}{$\sim$ 3368}                                                                                  & 128          & 1024          & 4096         \\ \midrule
% Bit Precision               & \multicolumn{1}{c|}{FP-32}                     & FP-32                        & \multicolumn{1}{c|}{FP-32}                        & FIX-8                                                                                       & FIX-16                                                                                        & \multicolumn{1}{c|}{-}                                                                                            & \multicolumn{3}{c}{FIX-16}                  \\ \midrule
% Test Network                & \multicolumn{9}{c}{Shallow Transformer}                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \midrule
% Latency (ms)                & \multicolumn{1}{c|}{2.17}                      & 16.24                        & \multicolumn{1}{c|}{1.70}                         & 0.30                                                                                        & 2.94                                                                                          & \multicolumn{1}{c|}{0.32}                                                                                         & 2.01         & 0.42          & 0.15         \\ \midrule
% Batch-1 Throughput (GOP/s)  & \multicolumn{1}{c|}{101.38}                    & 13.55                        & \multicolumn{1}{c|}{129.41}                       & 733.33                                                                                      & 75.34                                                                                         & \multicolumn{1}{c|}{687.50}                                                                                       & 109.45       & 523.81        & 1466.67      \\ \midrule
% Power (W)                   & \multicolumn{1}{c|}{165.00}                    & 7.56                         & \multicolumn{1}{c|}{250.00}                       & 16.70                                                                                       & 22.45                                                                                         & \multicolumn{1}{c|}{-}                                                                                            & 2.71         & 9.87          & 26.59        \\ \midrule
% Energy Efficiency (GOP/J)   & \multicolumn{1}{c|}{0.61}                      & 1.79                         & \multicolumn{1}{c|}{0.52}                         & 43.91                                                                                       & 3.35                                                                                          & \multicolumn{1}{c|}{-}                                                                                            & 40.39        & 53.07         & 55.16        \\ \midrule
% MAC Efficiency (GOP/s/unit) & \multicolumn{1}{c|}{-}                         & -                            & \multicolumn{1}{c|}{-}                            & 0.18                                                                                        & $\sim$ 0.01                                                                                   & \multicolumn{1}{c|}{$\sim$ 0.20}                                                                                  & 0.86         & 0.51          & 0.36         \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

\begin{table*}[ht]
\centering
\caption{\RoundOne{Comparison of STAs with previous works and commercial products}}
\label{tab:perf_cmp}
\resizebox{0.90\textwidth}{!}{%
\begin{tabular}{@{}c|cccccccccc@{}}
\toprule
\multirow{3}{*}{Platform}   & CPU                                            & \multicolumn{3}{|c}{GPU}                                                                                                                               & \multicolumn{6}{|c}{FPGA}                                                                                                                                                                                                                                                                                                                                 \\ \cmidrule(l){2-11} 
                            & \multicolumn{1}{c|}{\multirow{2}{*}{i9-9900X}} & \multirow{2}{*}{Jetson Nano} & \multirow{2}{*}{RTX 2080 Ti} & \multicolumn{1}{c|}{\multirow{2}{*}{\RoundOne{RTX 3090}}}                                          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SOCC'20\\ \cite{lu2020hardware}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ISLPED'20\\ \cite{li2020ftrans}\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ISQED'21\\ \cite{peng2021accelerating}\end{tabular}}} & \multicolumn{3}{c}{Our work}                \\ \cmidrule(l){9-11} 
                            & \multicolumn{1}{c|}{}                          &                              &                              & \multicolumn{1}{c|}{}                                                                   &                                                                                          &                                                                                          & \multicolumn{1}{c|}{}                                                                                                & STA-Tiny     & STA-Small     & STA-Large    \\ \midrule
Chip                        & \multicolumn{1}{c|}{Skylake}                   & Tegra X1                     & TU102                        & \multicolumn{1}{c|}{\RoundOne{GA102}}                                                              & XCVU13P                                                                                  & XCVU9P                                                                                   & \multicolumn{1}{c|}{XCU200}                                                                                          & XC7Z020      & XC7VX485T     & XCVU13P      \\ \midrule
Technology                  & \multicolumn{1}{c|}{14 nm}                     & 20 nm                        & 12 nm                        & \multicolumn{1}{c|}{\RoundOne{8 nm}}                                                               & 16 nm                                                                                    & 16 nm                                                                                    & \multicolumn{1}{c|}{16 nm}                                                                                           & 28 nm        & 28 nm         & 16 nm        \\ \midrule
Frequency                   & \multicolumn{1}{c|}{3.50 GHz}                  & 640 MHz                      & 1.35 GHz                     & \multicolumn{1}{c|}{\RoundOne{1.70 GHz}}                                                           & 200 MHz                                                                                  & -                                                                                        & \multicolumn{1}{c|}{-}                                                                                               & 150 MHz      & 200 MHz       & 200 MHz      \\ \midrule
Methods                     & \multicolumn{1}{c|}{-}                         & -                            & -                            & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\RoundOne{2:4 group-based} \\ \RoundOne{pruning}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Low-bit\\ quantization\end{tabular}                           & \begin{tabular}[c]{@{}c@{}}Block-circulant\\ matrix with FFT\end{tabular}                & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Block-based\\ pruning\end{tabular}}                                   & \multicolumn{3}{c}{N:M group-based pruning} \\ \midrule
\# MAC units                 & \multicolumn{1}{c|}{-}                         & -                            & -                            & \multicolumn{1}{c|}{\RoundOne{-}}                                                                  & 4096                                                                                     & $\sim$ 5647                                                                              & \multicolumn{1}{c|}{$\sim$ 3368}                                                                                     & 128          & 1024          & 4096         \\ \midrule
Bit Precision               & \multicolumn{1}{c|}{FP-32}                     & FP-32                        & FP-32                        & \multicolumn{1}{c|}{\RoundOne{FP-32}}                                                              & FIX-8                                                                                    & FIX-16                                                                                   & \multicolumn{1}{c|}{-}                                                                                               & \multicolumn{3}{c}{FIX-16}                  \\ \midrule
Test Network                & \multicolumn{10}{c}{Shallow Transformer}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \midrule
Latency (ms)                & \multicolumn{1}{c|}{2.17}                      & 16.24                        & 1.70                         & \multicolumn{1}{c|}{\RoundOne{0.46}}                                                               & 0.30                                                                                     & 2.94                                                                                     & \multicolumn{1}{c|}{0.32}                                                                                            & 2.01         & 0.42          & 0.15         \\ \midrule
Batch-1 Throughput (GOP/s)  & \multicolumn{1}{c|}{101.38}                    & 13.55                        & 129.41                       & \multicolumn{1}{c|}{\RoundOne{478.26}}                                                             & 733.33                                                                                   & 75.34                                                                                    & \multicolumn{1}{c|}{687.50}                                                                                          & 109.45       & 523.81        & 1466.67      \\ \midrule
Power (W)                   & \multicolumn{1}{c|}{165.00}                    & 7.56                         & 250.00                       & \multicolumn{1}{c|}{\RoundOne{350.00}}                                                             & 16.70                                                                                    & 22.45                                                                                    & \multicolumn{1}{c|}{-}                                                                                               & 2.71         & 9.87          & 26.59        \\ \midrule
Energy Efficiency (GOP/J)   & \multicolumn{1}{c|}{0.61}                      & 1.79                         & 0.52                         & \multicolumn{1}{c|}{\RoundOne{1.37}}                                                               & 43.91                                                                                    & 3.35                                                                                     & \multicolumn{1}{c|}{-}                                                                                               & 40.39        & 53.07         & 55.16        \\ \midrule
MAC Efficiency (GOP/s/unit) & \multicolumn{1}{c|}{-}                         & -                            & -                            & \multicolumn{1}{c|}{\RoundOne{-}}                                                                  & 0.18                                                                                     & $\sim$ 0.01                                                                              & \multicolumn{1}{c|}{$\sim$ 0.20}                                                                                                          & 0.86         & 0.51          & 0.36         \\ \bottomrule
\end{tabular}%
}
\end{table*}


% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table*}[ht]
% \centering
% \caption{\RoundOne{Comparison of STAs with previous works and commercial products}}
% \label{tab:perf_cmp}
% \resizebox{0.8\textwidth}{!}{%
% \begin{tabular}{@{}c|cccccccccc@{}}
% \toprule
% \multirow{3}{*}{Platform}   & CPU                                            & \multicolumn{3}{|c}{GPU}                                                                                                                               & \multicolumn{6}{|c}{FPGA}                                                                                                                                                                                                                                                                                                                                 \\ \cmidrule(l){2-11} 
%                             & \multicolumn{1}{c|}{\multirow{2}{*}{i9-9900X}} & \multirow{2}{*}{Jetson Nano} & \multirow{2}{*}{RTX 2080 Ti} & \multicolumn{1}{c|}{\multirow{2}{*}{RTX 3090}}                                          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SOCC'20\\ \cite{lu2020hardware}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ISLPED'20\\ \cite{li2020ftrans}\end{tabular}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ISQED'21\\ \cite{peng2021accelerating}\end{tabular}}} & \multicolumn{3}{c}{Our work}                \\ \cmidrule(l){9-11} 
%                             & \multicolumn{1}{c|}{}                          &                              &                              & \multicolumn{1}{c|}{}                                                                   &                                                                                          &                                                                                          & \multicolumn{1}{c|}{}                                                                                                & STA-Tiny     & STA-Small     & STA-Large    \\ \midrule
% Chip                        & \multicolumn{1}{c|}{Skylake}                   & Tegra X1                     & TU102                        & \multicolumn{1}{c|}{GA102}                                                              & XCVU13P                                                                                  & XCVU9P                                                                                   & \multicolumn{1}{c|}{XCU200}                                                                                          & XC7Z020      & XC7VX485T     & XCVU13P      \\ \midrule
% Technology                  & \multicolumn{1}{c|}{14 nm}                     & 20 nm                        & 12 nm                        & \multicolumn{1}{c|}{8 nm}                                                               & 16 nm                                                                                    & 16 nm                                                                                    & \multicolumn{1}{c|}{16 nm}                                                                                           & 28 nm        & 28 nm         & 16 nm        \\ \midrule
% Frequency                   & \multicolumn{1}{c|}{3.50 GHz}                  & 640 MHz                      & 1.35 GHz                     & \multicolumn{1}{c|}{1.70 GHz}                                                           & 200 MHz                                                                                  & -                                                                                        & \multicolumn{1}{c|}{-}                                                                                               & 150 MHz      & 200 MHz       & 200 MHz      \\ \midrule
% Methods                     & \multicolumn{1}{c|}{-}                         & -                            & -                            & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}2:4 group-based \\ pruning\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Low-bit\\ quantization\end{tabular}                           & \begin{tabular}[c]{@{}c@{}}Block-circulant\\ matrix with FFT\end{tabular}                & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Block-based\\ pruning\end{tabular}}                                   & \multicolumn{3}{c}{N:M group-based pruning} \\ \midrule
% \# MAC units                 & \multicolumn{1}{c|}{-}                         & -                            & -                            & \multicolumn{1}{c|}{-}                                                                  & 4096                                                                                     & $\sim$ 5647                                                                              & \multicolumn{1}{c|}{$\sim$ 3368}                                                                                     & 128          & 1024          & 4096         \\ \midrule
% Bit Precision               & \multicolumn{1}{c|}{FP-32}                     & FP-32                        & FP-32                        & \multicolumn{1}{c|}{FP-32}                                                              & FIX-8                                                                                    & FIX-16                                                                                   & \multicolumn{1}{c|}{-}                                                                                               & \multicolumn{3}{c}{FIX-16}                  \\ \midrule
% Test Network                & \multicolumn{10}{c}{Shallow Transformer}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \midrule
% Latency (ms)                & \multicolumn{1}{c|}{2.17}                      & 16.24                        & 1.70                         & \multicolumn{1}{c|}{0.46}                                                               & 0.30                                                                                     & 2.94                                                                                     & \multicolumn{1}{c|}{0.32}                                                                                            & 2.01         & 0.42          & 0.15         \\ \midrule
% Batch-1 Throughput (GOP/s)  & \multicolumn{1}{c|}{101.38}                    & 13.55                        & 129.41                       & \multicolumn{1}{c|}{478.26}                                                             & 733.33                                                                                   & 75.34                                                                                    & \multicolumn{1}{c|}{687.50}                                                                                          & 109.45       & 523.81        & 1466.67      \\ \midrule
% Power (W)                   & \multicolumn{1}{c|}{165.00}                    & 7.56                         & 250.00                       & \multicolumn{1}{c|}{350.00}                                                             & 16.70                                                                                    & 22.45                                                                                    & \multicolumn{1}{c|}{-}                                                                                               & 2.71         & 9.87          & 26.59        \\ \midrule
% Energy Efficiency (GOP/J)   & \multicolumn{1}{c|}{0.61}                      & 1.79                         & 0.52                         & \multicolumn{1}{c|}{1.37}                                                               & 43.91                                                                                    & 3.35                                                                                     & \multicolumn{1}{c|}{-}                                                                                               & 40.39        & 53.07         & 55.16        \\ \midrule
% MAC Efficiency (GOP/s/unit) & \multicolumn{1}{c|}{-}                         & -                            & -                            & \multicolumn{1}{c|}{-}                                                                  & 0.18                                                                                     & $\sim$ 0.01                                                                              & \multicolumn{1}{c|}{$\sim$ 0.20}                                                                                                         & 0.86         & 0.51          & 0.36         \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

Finally, we compare STA with other previous FPGA-based works and commercial CPU and GPU products.
Table~\ref{tab:perf_cmp} presents a fair performance comparison without batching on various platforms.
Prior FPGA-based works for accelerating Transformers, include \cite{lu2020hardware}, \cite{li2020ftrans}, and \cite{peng2021accelerating}.
The dedicated accelerator in \cite{lu2020hardware}, equipped with a large 2D systolic array for dense operation, is the pioneer work for Transformer acceleration.
FTRANS \cite{li2020ftrans}, is another recent specialized accelerator for Transformers, which exploits the speedup potential of block-circulant weight representations.
In \cite{peng2021accelerating}, the proposed accelerator utilizes coarse-grained block-based sparsity to speedup Transformer inference.
% The shallow Transformer are used as a benchmark for these computing systems.
The shallow Transformer used in \cite{li2020ftrans} and \cite{peng2021accelerating} is applied as a benchmark for a fair evaluation.
% It has two encoder layers and one decoder layer with an embedding layer size of 800 and a number of 200 as the hidden layer dimension. 
The comparison is benchmarked on CPU, GPUs, prior cutting-edge FPGA solutions, and STA on various FPGA platforms.
We evaluate these designs in terms of latency, throughput, power, energy efficiency, and MAC efficiency.
All of them are key metrics for a computing system.

As shown in Table~\ref{tab:perf_cmp}, STA-Tiny far outperforms the embedded GPU, Jetson Nano, and the high-end CPU, i9-9900X, in all evaluated metrics.
STA-Small surpasses the CPU and GPU platforms in all metrics.
Moreover, STA-Small is close to \cite{lu2020hardware} and \cite{peng2021accelerating} in terms of latency and throughput, while using a relatively small number of MACs compared to them.
The energy efficiency and MAC efficiency of STA-Small are also superior to all previous FPGA-based works.
% STA-Large, having similar peak performance in the core computing engine, achieves significant improvements over all prior FPGA platforms in all evaluated metrics.
Compared to previous FPGA solutions, STA-Large achieves $2.00 \sim 19.47 \times$ throughput improvement, achieves $1.26 \sim 16.47 \times$ energy efficiency improvement, and $1.80 \sim 36.00\times$ MAC efficiency gain, respectively.
The performance gain of STA comes from optimizations from two levels.
% At the algorithm level, the \textit{N:M} sparsity pattern is carefully considered, which can greatly reduce the computational cost of Transformer-based models.
At the algorithm level, we carefully exploit the potential of \textit{N:M} sparsity pattern, which can significantly reduce the computational cost of Transformer-based models.
At the hardware level, STA can efficiently handle \textit{N:M} sparse parameters, which significantly improves the utilization of computing units.
In addition, our deployment framework, taking STA-Tiny, STA-Small, and STA-Large as examples, can realize flexible hardware generation for Transformers.
The proposed framework can flexibly and efficiently meet the requirements for deploying Transformer-based models on various FPGA devices.


% [Note] Chao Fang: 这句话应该怎么说好呢
% Based on the computational capabilities of STAs, the evaluation is divided into two parts, namely edge and cloud.

% \subsection{Eval. V: System Speedup on Various Transformer-based Models}
% \subsection{Eval. VI: Framework Flexibility on Various FPGA Platforms}
% \subsection{Eval. VII: Comparison of Our System with the State-of-the-art Works and Commercial Products}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}

